Next-to-next-to-leading order ${\cal O}(\alpha_s^4)$ results for heavy quark pair production in quark--antiquark collisions: The one-loop squared contributions

We calculate the next-to-next-to-leading order ${\cal O}(\alpha_s^4)$ one-loop squared corrections to the production of heavy quark pairs in quark-antiquark annihilations. These are part of the next-to-next-to-leading order ${\cal O}(\alpha_s^4)$ radiative QCD corrections to this process. Our results, with the full mass dependence retained, are presented in a closed and very compact form, in the dimensional regularization scheme. We have found very intriguing factorization properties for the finite part of the amplitudes.

==> rfull <==
%auto-ignore
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%    NNLO ${\cal O}(\alpha_s^4)$ results for heavy quark pair production in 
5       quark--antiquark collisions: The one-loop squared contributions
%
% This file in REDUCE format (compressed) is full result for the squared
% matrix element, Eq. (4.1). Other formats are also available upon request.
%
%                      Definitions:
%  eps = 1/eps,  eps2 = 1/eps^2,  eps3 = 1/eps^3,  eps4 = 1/eps^4;
%  nlf  is the number of light flavors;
%  ln = ln(-t/m^2),  lnu = ln(-u/m^2);
%  nc = 3, cf = 4/3 - color factors defined in the paper;


full := ( - 4*((((2*(3*(((3*(2*(((3*((4*(3*((t**3 + 3*t**2*u + 3*t*u**2 + u**3)*
m**2 + (t**2 + 2*t*u + u**2)*t*u)*nc - (2*t + 7*u + 18*m**2)*(t**3 + 3*t**2*u + 
3*t*u**2 + u**3))*m**2 - (2*(2*t + 7*u + 18*m**2)*(t**4 + 4*t**3*u + 6*t**2*u**2
 + 4*t*u**3 + u**4) + 3*(t**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 
+ u**5)*nc))*eps - ((7*t - 11*u - 8*m**2)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u
**3 + u**4) - 3*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5
)*nc + 2*((7*t - 11*u - 8*m**2)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3) - 3*(t**4 + 
4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*nc)*m**2))*(t + u)*b5(0)*c6(-1)*t*u + 
4*((2*((14*nc + nlf)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*t*u - (6*
t**6 + 50*t**5*u + 161*t**4*u**2 + 264*t**3*u**3 + 236*t**2*u**4 + 110*t*u**5 + 
21*u**6))*m**2 - (nlf + 1 + 14*nc)*(t**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 
+ 3*t*u**4 + u**5)*t*u)*eps + (nlf + 1 + 14*nc)*(t**5 + 5*t**4*u + 10*t**3*u**2 
+ 10*t**2*u**3 + 5*t*u**4 + u**5)*t*u + 3*(2*t**6 + 31*t**5*u + 125*t**4*u**2 + 
230*t**3*u**3 + 220*t**2*u**4 + 107*t*u**5 + 21*u**6)*m**2)*(t + u + 4*m**2)*c4(
-1))*(2*cf - nc) - 2*(2*((t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4 - 2*(t
**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2)*(7*ln + 2*lnu)*(5*nc - 2*nlf)*eps - (35*
ln*nc - 14*ln*nlf + 60*ln + 10*lnu*nc - 4*lnu*nlf + 12*lnu)*(t**4 + 4*t**3*u + 6
*t**2*u**2 + 4*t*u**3 + u**4)) + 135*((t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 
+ u**4 - 2*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2)*eps - (t**4 + 4*t**3*u + 6*
t**2*u**2 + 4*t*u**3 + u**4))*cf**2 + 3*((12*lnu + 25*nc - 10*nlf + 40 + 42*ln)*
(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4) - (12*lnu + 25*nc - 10*nlf + 
42*ln)*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4 - 2*(t**3 + 3*t**2*u + 3
*t*u**2 + u**3)*m**2)*eps)*cf)*(t + u + 4*m**2)*b5(0)*t*u + 6*(((2*(nlf - 4) - 5
*nc)*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5) + (t**5 +
 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5 - 2*(t**4 + 4*t**3*u + 6
*t**2*u**2 + 4*t*u**3 + u**4)*m**2)*(5*nc - 2*nlf)*eps)*nc + 18*((t**5 + 3*t**4*
u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5 - 2*(t**4 + 4*t**3*u + 6*t**2*u
**2 + 4*t*u**3 + u**4)*m**2)*eps - (t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**
3 + 5*t*u**4 + u**5))*cf**2 - ((4*(nlf - 4) - 19*nc)*(t**5 + 5*t**4*u + 10*t**3*
u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5) + (t**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2
*u**3 + 3*t*u**4 + u**5 - 2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m
**2)*(19*nc - 4*nlf)*eps)*cf)*(t + u + 4*m**2)*b5(0)*c4(-1)*t*u - 6*(((4*nlf + 
27 - 19*nc)*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4 - 2*(t**3 + 3*t**2*
u + 3*t*u**2 + u**3)*m**2)*eps2 - (4*nlf + 11 - 19*nc)*(t**4 + 4*t**3*u + 6*t**2
*u**2 + 4*t*u**3 + u**4)*eps + 18*((t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u
**4 - 2*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2)*eps2 - (t**4 + 4*t**3*u + 6*t
**2*u**2 + 4*t*u**3 + u**4)*eps)*cf)*cf - ((6*(nlf - 4) + 5*nc**2 - (2*nlf + 7)*
nc)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*eps - (5*nc**2 + 6*nlf - (
2*nlf + 15)*nc)*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4 - 2*(t**3 + 3*t
**2*u + 3*t*u**2 + u**3)*m**2)*eps2))*(t + u + 4*m**2)*b5(0)*t*u + 4*((2*(2*(14*
nc + nlf)*(t**2 + 2*t*u + u**2)*t**2*u**2 - (6*t**6 + 51*t**5*u + 163*t**4*u**2 
+ 266*t**3*u**3 + 238*t**2*u**4 + 111*t*u**5 + 21*u**6))*m**2 - (nlf + 1 + 14*nc
)*(t**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5)*t*u + 4*((14*
nc + nlf)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*t*u - (6*t**5 + 44*t**4*u + 117*t
**3*u**2 + 147*t**2*u**3 + 89*t*u**4 + 21*u**5))*m**4)*eps + (nlf + 1 + 14*nc)*(
t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)*t*u + 6*(2*t**5
 + 29*t**4*u + 96*t**3*u**2 + 134*t**2*u**3 + 86*t*u**4 + 21*u**5)*m**4 + (2*(14
*nc + nlf)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*t*u + 6*t**6 + 95*t
**5*u + 383*t**4*u**2 + 702*t**3*u**3 + 668*t**2*u**4 + 323*t*u**5 + 63*u**6)*m
**2)*(t + u + 4*m**2)*(2*cf - nc)*c6(-1) - 6*((((2*m**2 + u)*t**2 + 12*(m**2 + u
)*u**2 + 2*(4*m**2 + 3*u)*t*u)*t**2 + ((10*t + 3*u)*u + 2*(4*t + u)*m**2)*u**3)*
eps - 2*(((t + u)*m**2 + t*u)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3) + (t**4 + 4*t
**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2)*eps2)*(nc - 3 - 2*cf)*(t + u + 4*m
**2)*b1u(0)*t)*((t + u)*m**2 + t*u) - 6*((2*((6*m**2*u - t**2 + 2*(m**2 - u)*t)*
t**2 + (2*(3*m**2 + u)*t + (2*m**2 + u)*u)*u**2)*eps2 + (3*t**4 + 8*t**3*u + 6*t
**2*u**2 - u**4)*eps)*((t + u)*m**2 + t*u) - (3*(t**5 + 5*t**4*u + 10*t**3*u**2 
+ 10*t**2*u**3 + 5*t*u**4 + u**5) - 2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 
+ u**4)*eps*t)*u)*(nc - 3 - 2*cf)*(t + u + 4*m**2)*c3u(0)*t*u**2 - 21*((2*((6*(t
 - u + m**2)*u + (t - 4*u + 2*m**2)*t)*t**2 + (6*t**2 - 2*t*u - u**2 + 2*(3*t + 
u)*m**2)*u**2)*eps2 + (5*t**4 + 16*t**3*u + 18*t**2*u**2 + 8*t*u**3 + u**4)*eps)
*((t + u)*m**2 + t*u) - (2*(2*t**5 + 9*t**4*u + 16*t**3*u**2 + 14*t**2*u**3 + 6*
t*u**4 + u**5)*eps - 3*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4
 + u**5))*t)*(nc - 3 - 2*cf)*(t + u + 4*m**2)*c3(0)*t**2*u) + 3*(2*(8*(3*(t**3 +
 3*t**2*u + 3*t*u**2 + u**3)*nc + 10*(t**2 + 2*t*u + u**2)*(t - u))*m**6 - 5*(t
**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)*(t - u) + 8*(5*(
t**3 + 3*t**2*u + 3*t*u**2 + u**3)*(t - u) + 3*(t**2 + 2*t*u + u**2)*nc*t*u)*m**
4 - 2*(3*(t**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5)*nc + 5*
(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*(t - u))*m**2)*eps - (8*(2*(7*
t**4 + 19*t**3*u + 15*t**2*u**2 + t*u**3 - 2*u**4) - 3*(t**4 + 4*t**3*u + 6*t**2
*u**2 + 4*t*u**3 + u**4)*nc)*m**4 + 5*(t**6 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*
u**3 + 15*t**2*u**4 + 6*t*u**5 + u**6) + 6*(11*t**5 + 43*t**4*u + 62*t**3*u**2 +
 38*t**2*u**3 + 7*t*u**4 - u**5 - 2*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u
**3 + 5*t*u**4 + u**5)*nc)*m**2))*((t + u)*m**2 + t*u)*(2*cf - nc)*(t + u)*c1(0)
*c6(-1)*t*u - 12*((2*(3*((t**3 + 3*t**2*u + 3*t*u**2 + u**3)*nc**2 + 10*(t**2 + 
2*t*u + u**2)*(t - u)) - (19*t**3 + 37*t**2*u + 17*t*u**2 - u**3)*nc)*m**2 - 3*(
nc - 3)*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4)*nc)*eps2 + 3*(((t**4 +
 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*nc + 12*(t**2 + 2*t*u + u**2)*(t - u)
*m**2)*eps - 8*((t + u)*m**2 + t*u)*(t + u)*eps2*m**2*nc)*(nc - 3) + 2*(3*(8*(2*
nc - 3 - 2*cf)*((t + u)*m**2 + t*u)*(t + u)*eps2*m**2 - ((t**4 + 4*t**3*u + 6*t
**2*u**2 + 4*t*u**3 + u**4)*nc + 12*(t**2 + 2*t*u + u**2)*(t - u)*m**2)*eps) - (
2*(3*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*nc - 10*(t**2 + 2*t*u + u**2)*(t - u))*
m**2 - 3*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4)*nc)*eps2)*cf)*((t + u
)*m**2 + t*u)*(t + u)*t*u - 12*(((4*((t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2 + 
(t**2 + 2*t*u + u**2)*t*u)*m**2 - (t**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 +
 3*t*u**4 + u**5))*(5*nc - 2*nlf)*eps - (2*(nlf - 4) - 5*nc)*(t**5 + 5*t**4*u + 
10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5 + 2*(t**4 + 4*t**3*u + 6*t**2*u**2
 + 4*t*u**3 + u**4)*m**2))*nc + 18*((4*((t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2
 + (t**2 + 2*t*u + u**2)*t*u)*m**2 - (t**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**
3 + 3*t*u**4 + u**5))*eps + t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*
u**4 + u**5 + 2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2)*cf**2 - 
((4*((t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2 + (t**2 + 2*t*u + u**2)*t*u)*m**2 
- (t**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5))*(19*nc - 4*
nlf)*eps - (4*(nlf - 4) - 19*nc)*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 
+ 5*t*u**4 + u**5 + 2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2))*
cf)*((t + u)*m**2 + t*u)*(t + u + 4*m**2)*b5(0)*c6(-1)*t*u + 6*(5*((3*(t**4 + 2*
t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4 - 2*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m
**2)*nc + 2*(2*t + 7*u + 18*m**2)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3))*eps + (7*
t - 11*u - 8*m**2)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3) - 3*(t**4 + 4*t**3*u + 6*
t**2*u**2 + 4*t*u**3 + u**4)*nc)*cf - 2*(((19*t - 23*u - 8*m**2)*(t**3 + 3*t**2*
u + 3*t*u**2 + u**3) - 7*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*nc)*
ln + 2*((t - 5*u - 8*m**2)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3) - (t**4 + 4*t**3*
u + 6*t**2*u**2 + 4*t*u**3 + u**4)*nc)*lnu) - 2*((7*(t**4 + 2*t**3*u + 2*t**2*u
**2 + 2*t*u**3 + u**4 - 2*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2)*nc + 2*(2*t 
+ 19*u + 42*m**2)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3))*ln + 2*((t**4 + 2*t**3*u 
+ 2*t**2*u**2 + 2*t*u**3 + u**4 - 2*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2)*nc
 + 2*(2*t + u + 6*m**2)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3))*lnu)*eps)*((t + u)*
m**2 + t*u)*(t + u)*b5(0)*t*u + 12*((15*((t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u
**3 + u**4)*nc + 12*(t**2 + 2*t*u + u**2)*(t - u)*m**2 + 16*((t + u)*m**2 + t*u)
*(t + u)*cf*eps*m**2) - 8*(8*lnu + 15*nc + 28*ln)*((t + u)*m**2 + t*u)*(t + u)*
eps*m**2 + 5*(2*(3*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*nc - 10*(t**2 + 2*t*u + u
**2)*(t - u))*m**2 - 3*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4)*nc)*eps
)*cf - 2*(((2*(7*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*nc - 34*(t**2 + 2*t*u + u**
2)*(t - u))*m**2 - 7*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4)*nc)*ln + 
2*(2*((t**3 + 3*t**2*u + 3*t*u**2 + u**3)*nc + 2*(t**2 + 2*t*u + u**2)*(t - u))*
m**2 - (t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4)*nc)*lnu)*eps + ((t**4 +
 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*nc + 12*(t**2 + 2*t*u + u**2)*(t - u)
*m**2 - 8*((t + u)*m**2 + t*u)*(t + u)*eps*m**2*nc)*(7*ln + 2*lnu)))*((t + u)*m
**2 + t*u)*(t + u)*t*u + 12*(3*((2*(2*(t**4 + 6*t**3*u + 10*t**2*u**2 + 6*t*u**3
 + u**4 + 2*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2)*m**2 - (t**5 + t**4*u - 2*
t**3*u**2 - 2*t**2*u**3 + t*u**4 + u**5))*m**2 - (t**6 + 4*t**5*u + 7*t**4*u**2 
+ 8*t**3*u**3 + 7*t**2*u**4 + 4*t*u**5 + u**6))*eps + 4*(t**5 + 5*t**4*u + 10*t
**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5 + (t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t
*u**3 + u**4)*m**2)*m**2 + t**6 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*u**3 + 15*t
**2*u**4 + 6*t*u**5 + u**6)*(4*cf**2 - 4*cf*nc + nc**2)*c6(-1) - ((4*((t**3 + 3*
t**2*u + 3*t*u**2 + u**3)*m**2 + (t**2 + 2*t*u + u**2)*t*u)*m**2 - (t**5 + 3*t**
4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5))*eps + t**5 + 5*t**4*u + 10*t
**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5 + 2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4
*t*u**3 + u**4)*m**2)*(2*((7*ln + 2*lnu)*nc + 15*cf**2) - (8*lnu + 15*nc + 28*ln
)*cf))*((t + u)*m**2 + t*u)*(t + u + 4*m**2)*c6(0)*t*u + 3*(2*(((4*(2*(7*t**4 + 
19*t**3*u + 15*t**2*u**2 + t*u**3 - 2*u**4) - 3*(t**4 + 4*t**3*u + 6*t**2*u**2 +
 4*t*u**3 + u**4)*nc)*m**2 + 5*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 
5*t*u**4 + u**5))*eps + 2*(5*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*(
t - u) + 6*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4)*m**2*nc - 4*(3*(t**
3 + 3*t**2*u + 3*t*u**2 + u**3)*nc + 10*(t**2 + 2*t*u + u**2)*(t - u))*m**4)*
eps2)*cf + (4*((t**3 - 17*t**2*u - 37*t*u**2 - 19*u**3)*nc - 30*(t**2 + 2*t*u + 
u**2)*(t - u) + 3*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*nc**2)*m**4 - (5*(t**4 + 4
*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*(t - u) + 6*(t**4 + 2*t**3*u + 2*t**2*u
**2 + 2*t*u**3 + u**4)*m**2*nc)*(nc - 3))*eps2) + (4*(3*(2*(7*t**4 + 19*t**3*u +
 15*t**2*u**2 + t*u**3 - 2*u**4) + (t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u
**4)*nc**2) - (23*t**4 + 74*t**3*u + 84*t**2*u**2 + 38*t*u**3 + 5*u**4)*nc)*m**2
 - 5*(nc - 3)*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5))
*eps)*((t + u)*m**2 + t*u)*(t + u)*c1(0)*t*u - 6*(((2*(8*t**4 + 23*t**3*u + 21*t
**2*u**2 + 5*t*u**3 - u**4 - 4*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2) - 3*(t
**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*nc)*nc - 3*(7*t - 11*u - 8*m**2)
*(t**3 + 3*t**2*u + 3*t*u**2 + u**3))*eps - 2*((3*(t**4 + 2*t**3*u + 2*t**2*u**2
 + 2*t*u**3 + u**4 - 2*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2)*nc + 2*(2*t + 7
*u + 18*m**2)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3))*eps2 + ((7*t - 11*u - 8*m**2)
*(t**3 + 3*t**2*u + 3*t*u**2 + u**3) - 3*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u
**3 + u**4)*nc)*eps)*cf - ((((5*t + 4*u - 36*m**2)*t**2 - 12*(t + 2*u + 9*m**2)*
(t + u)*u)*t - (4*t + 5*u + 36*m**2)*u**3)*nc + 3*((2*(nc - 3)*(t**3 + 3*t**2*u 
+ 3*t*u**2 + u**3)*m**2 - (t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4)*nc)*
nc + 2*(2*t + 7*u + 18*m**2)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)))*eps2)*((t + u
)*m**2 + t*u)*(t + u)*b5(0)*t*u - 3*(2*((4*(2*(19*t**4 + 55*t**3*u + 51*t**2*u**
2 + 13*t*u**3 - 2*u**4) - 7*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*nc
)*m**2 + 17*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5))*
ln - 2*(4*((t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*nc - 2*(t**4 + t**3
*u - 3*t**2*u**2 - 5*t*u**3 - 2*u**4))*m**2 + t**5 + 5*t**4*u + 10*t**3*u**2 + 
10*t**2*u**3 + 5*t*u**4 + u**5)*lnu + 2*((17*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*
t*u**3 + u**4)*(t - u) + 14*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4)*m
**2*nc - 4*(7*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*nc + 34*(t**2 + 2*t*u + u**2)*
(t - u))*m**4)*ln - 2*((t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*(t - u)
 - 2*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4)*m**2*nc + 4*((t**3 + 3*t
**2*u + 3*t*u**2 + u**3)*nc - 2*(t**2 + 2*t*u + u**2)*(t - u))*m**4)*lnu)*eps) -
 5*(4*(2*(7*t**4 + 19*t**3*u + 15*t**2*u**2 + t*u**3 - 2*u**4) - 3*(t**4 + 4*t**
3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*nc)*m**2 + 5*(t**5 + 5*t**4*u + 10*t**3*u**
2 + 10*t**2*u**3 + 5*t*u**4 + u**5) + 2*(5*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*
u**3 + u**4)*(t - u) + 6*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4)*m**2*
nc - 4*(3*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*nc + 10*(t**2 + 2*t*u + u**2)*(t -
 u))*m**4)*eps)*cf)*((t + u)*m**2 + t*u)*(t + u)*c1(0)*t*u - 12*(((3*(t**5 + 3*t
**4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5 + 8*(t**3 + 3*t**2*u + 3*t*u
**2 + u**3)*m**4)*nc + 2*(10*(t**4 + 2*t**3*u - 2*t*u**3 - u**4) - 3*(t**4 - 2*t
**2*u**2 + u**4)*nc)*m**2)*eps - 3*((t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u
**3 + 5*t*u**4 + u**5)*nc + 12*(t**4 + 2*t**3*u - 2*t*u**3 - u**4)*m**2))*nc + 
96*((t + u)*m**2 + t*u)*(t**2 + 2*t*u + u**2)*cf**2*eps*m**2 + 2*(3*((t**5 + 5*t
**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)*nc + 12*(t**3 + 3*t**2*u 
+ 3*t*u**2 + u**3)*(t - u)*m**2 - 16*((t + u)*m**2 + t*u)*(t**2 + 2*t*u + u**2)*
eps*m**2*nc) + (2*(3*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*nc - 10*(
t**3 + 3*t**2*u + 3*t*u**2 + u**3)*(t - u))*m**2 - 3*(t**5 + 3*t**4*u + 4*t**3*u
**2 + 4*t**2*u**3 + 3*t*u**4 + u**5)*nc)*eps)*cf)*((t + u)*m**2 + t*u)*(t + u)*
c4(-1)*t*u - 12*(2*(3*((t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4
 + u**5)*nc + 24*(t**2 + 2*t*u + u**2)*(t - u)*m**4 + 16*(t**2 + 2*t*u + u**2 + 
2*(t + u)*m**2)*((t + u)*m**2 + t*u)*(cf - nc)*eps*m**2 + 2*((t**4 + 4*t**3*u + 
6*t**2*u**2 + 4*t*u**3 + u**4)*nc + 6*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*(t - u
))*m**2) + (4*(3*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*nc - 10*(t**2 + 2*t*u + u**
2)*(t - u))*m**4 - 3*(t**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u
**5)*nc - 4*(5*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*(t - u) - 3*(t**2 + 2*t*u + u
**2)*nc*t*u)*m**2)*eps)*cf - (3*((t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 
+ 5*t*u**4 + u**5)*nc + 24*(t**2 + 2*t*u + u**2)*(t - u)*m**4 - 8*(t**2 + 2*t*u 
+ u**2 + 2*(t + u)*m**2)*((t + u)*m**2 + t*u)*eps*m**2*nc + 2*((t**4 + 4*t**3*u 
+ 6*t**2*u**2 + 4*t*u**3 + u**4)*nc + 6*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*(t -
 u))*m**2) + (4*(3*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*nc - 10*(t**2 + 2*t*u + u
**2)*(t - u))*m**4 - 3*(t**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 +
 u**5)*nc - 4*(5*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*(t - u) - 3*(t**2 + 2*t*u +
 u**2)*nc*t*u)*m**2)*eps)*nc)*((t + u)*m**2 + t*u)*(t + u)*c6(-1)*t*u + 6*(5*(2*
(7*t**5 + 37*t**4*u + 78*t**3*u**2 + 82*t**2*u**3 + 43*t*u**4 + 9*u**5 - 10*(t**
4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2 - 2*(7*t**5 + 21*t**4*u + 23*
t**3*u**2 + 13*t**2*u**3 + 6*t*u**4 + 2*u**5)*eps)*((t + u)*m**2 + t*u) + (5*t**
6 + 34*t**5*u + 95*t**4*u**2 + 140*t**3*u**3 + 115*t**2*u**4 + 50*t*u**5 + 9*u**
6)*m**2 + 14*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*t**3)*cf - 2*(((
17*t**6 + 106*t**5*u + 275*t**4*u**2 + 380*t**3*u**3 + 295*t**2*u**4 + 122*t*u**
5 + 21*u**6)*m**2 + 38*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*t**3)*
ln - 2*((t**6 + 2*t**5*u - 5*t**4*u**2 - 20*t**3*u**3 - 25*t**2*u**4 - 14*t*u**5
 - 3*u**6)*m**2 - 2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*t**3)*lnu)
 - 4*((19*t**5 + 97*t**4*u + 198*t**3*u**2 + 202*t**2*u**3 + 103*t*u**4 + 21*u**
5 - 34*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2)*ln + 2*(t**5 + 7*
t**4*u + 18*t**3*u**2 + 22*t**2*u**3 + 13*t*u**4 + 3*u**5 + 2*(t**4 + 4*t**3*u +
 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2)*lnu - 2*((19*t**5 + 57*t**4*u + 59*t**3*u
**2 + 25*t**2*u**3 + 6*t*u**4 + 2*u**5)*ln + 2*(t**5 + 3*t**4*u + 5*t**3*u**2 + 
7*t**2*u**3 + 6*t*u**4 + 2*u**5)*lnu)*eps)*((t + u)*m**2 + t*u))*(t + u + 4*m**2
)*c1(0)*t*u - 8*(2*((2*((14*nc + nlf)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*t*u - 
(6*t**5 + 44*t**4*u + 117*t**3*u**2 + 147*t**2*u**3 + 89*t*u**4 + 21*u**5))*m**2
 - (nlf + 1 + 14*nc)*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4)*t*u)*eps2
 + ((nlf + 1 + 14*nc)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*t*u + 3*
(2*t**5 + 29*t**4*u + 96*t**3*u**2 + 134*t**2*u**3 + 86*t*u**4 + 21*u**5)*m**2)*
eps)*cf - (((nlf - 41 + 14*nc)*nc - 3*(nlf + 1))*(t**4 + 4*t**3*u + 6*t**2*u**2 
+ 4*t*u**3 + u**4)*t*u + 3*(nc - 3)*(2*t**5 + 29*t**4*u + 96*t**3*u**2 + 134*t**
2*u**3 + 86*t*u**4 + 21*u**5)*m**2)*eps - (2*((14*nc**2 - 3*nlf)*(t**3 + 3*t**2*
u + 3*t*u**2 + u**3)*t*u + 3*(6*t**5 + 44*t**4*u + 117*t**3*u**2 + 147*t**2*u**3
 + 89*t*u**4 + 21*u**5) - (6*t**5 + 86*t**4*u + 243*t**3*u**2 + 273*t**2*u**3 + 
131*t*u**4 + 21*u**5 - (t**3 + 3*t**2*u + 3*t*u**2 + u**3)*nlf*t*u)*nc)*m**2 - (
(nlf - 41 + 14*nc)*nc - 3*(nlf + 1))*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 +
 u**4)*t*u)*eps2)*((t + u)*m**2 + t*u)*(t + u + 4*m**2)) - 8*(15*((2*((14*nc + 
nlf)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*t*u - (6*t**5 + 44*t**4*u + 117*t**3*u
**2 + 147*t**2*u**3 + 89*t*u**4 + 21*u**5))*m**2 - (nlf + 1 + 14*nc)*(t**4 + 2*t
**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4)*t*u)*eps + (nlf + 1 + 14*nc)*(t**4 + 4*t
**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*t*u + 3*(2*t**5 + 29*t**4*u + 96*t**3*u**
2 + 134*t**2*u**3 + 86*t*u**4 + 21*u**5)*m**2)*cf - 2*((7*(nlf + 1 + 14*nc)*(t**
4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*t*u + 9*(2*t**5 + 65*t**4*u + 240*
t**3*u**2 + 350*t**2*u**3 + 230*t*u**4 + 57*u**5)*m**2)*ln + 2*((nlf + 1 + 14*nc
)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*t*u + 9*(2*t**5 + 11*t**4*u 
+ 24*t**3*u**2 + 26*t**2*u**3 + 14*t*u**4 + 3*u**5)*m**2)*lnu) - 2*((2*(7*(14*nc
 + nlf)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*t*u - (18*t**5 + 236*t**4*u + 771*t
**3*u**2 + 1077*t**2*u**3 + 695*t*u**4 + 171*u**5))*m**2 - 7*(nlf + 1 + 14*nc)*(
t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4)*t*u)*ln + 2*(2*((14*nc + nlf)*(
t**3 + 3*t**2*u + 3*t*u**2 + u**3)*t*u - (18*t**5 + 80*t**4*u + 141*t**3*u**2 + 
123*t**2*u**3 + 53*t*u**4 + 9*u**5))*m**2 - (nlf + 1 + 14*nc)*(t**4 + 2*t**3*u +
 2*t**2*u**2 + 2*t*u**3 + u**4)*t*u)*lnu)*eps)*((t + u)*m**2 + t*u)*(t + u + 4*m
**2) - 126*((3*(2*m**2 + t)*(4*t + u)*u**3 - 2*t**5 + 3*(t - 2*u + 2*m**2)*t**4 
+ 6*(2*t - u + 4*m**2)*t**3*u + 2*(9*t - u + 18*m**2)*t**2*u**2)*eps - 2*(((t + 
u)*m**2 + t*u)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3) + (t**4 + 4*t**3*u + 6*t**2*u
**2 + 4*t*u**3 + u**4)*m**2)*eps2)*(nc - 3 - 2*cf)*((t + u)*m**2 + t*u)*(t + u +
 4*m**2)*b1(0)*u + 9*(2*(3*(12*((t + u)*m**2 + t*u)**2*(t**3 + 3*t**2*u + 3*t*u
**2 + u**3)*eps2 - (7*t**7 + 40*t**6*u + 93*t**5*u**2 + 110*t**4*u**3 + 65*t**3*
u**4 + 12*t**2*u**5 - 5*t*u**6 - 2*u**7)) + 2*(7*(2*t**6 + 11*t**5*u + 25*t**4*u
**2 + 30*t**3*u**3 + 20*t**2*u**4 + 7*t*u**5 + u**6)*t + 2*(t**6 + 6*t**5*u + 15
*t**4*u**2 + 20*t**3*u**3 + 15*t**2*u**4 + 6*t*u**5 + u**6)*m**2)*eps + 24*((t**
5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5 - 2*(t**4 + 4*t**3*u 
+ 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2)*eps2 - (t**5 + 5*t**4*u + 10*t**3*u**2 + 
10*t**2*u**3 + 5*t*u**4 + u**5)*eps)*((t + u)*m**2 + t*u)*cf - (2*(5*t**5 + 33*t
**4*u + 64*t**3*u**2 + 44*t**2*u**3 + 3*t*u**4 - 5*u**5 + 12*(t**5 + 3*t**4*u + 
4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5)*nc - 12*(2*nc - 3)*(t**4 + 4*t**3*u
 + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2)*eps2 + 3*(3*(5*t**5 + 21*t**4*u + 34*t**
3*u**2 + 26*t**2*u**3 + 9*t*u**4 + u**5) - 8*(t**5 + 5*t**4*u + 10*t**3*u**2 + 
10*t**2*u**3 + 5*t*u**4 + u**5)*nc)*eps)*((t + u)*m**2 + t*u))*cf - ((2*(3*(4*(
nc - 3)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2*nc + 23*t**5 + 87
*t**4*u + 136*t**3*u**2 + 116*t**2*u**3 + 57*t*u**4 + 13*u**5) - (5*t**5 + 33*t
**4*u + 64*t**3*u**2 + 44*t**2*u**3 + 3*t*u**4 - 5*u**5 + 6*(t**5 + 3*t**4*u + 4
*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5)*nc)*nc)*eps2 + 3*(4*(t**5 + 5*t**4*u
 + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)*nc**2 + 9*(t**5 + t**4*u - 6*t
**3*u**2 - 14*t**2*u**3 - 11*t*u**4 - 3*u**5) - 3*(5*t**5 + 21*t**4*u + 34*t**3*
u**2 + 26*t**2*u**3 + 9*t*u**4 + u**5)*nc)*eps)*((t + u)*m**2 + t*u) + (3*(12*((
t + u)*m**2 + t*u)**2*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*eps2 - (7*t**7 + 40*t
**6*u + 93*t**5*u**2 + 110*t**4*u**3 + 65*t**3*u**4 + 12*t**2*u**5 - 5*t*u**6 - 
2*u**7)) + 2*(7*(2*t**6 + 11*t**5*u + 25*t**4*u**2 + 30*t**3*u**3 + 20*t**2*u**4
 + 7*t*u**5 + u**6)*t + 2*(t**6 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*u**3 + 15*t
**2*u**4 + 6*t*u**5 + u**6)*m**2)*eps)*(nc - 3)))*(t + u + 4*m**2)*c4(0)*t*u - 
36*(((2*((2*(4*m**2 - u)*t**3 + (2*m**2 + u)*u**3 + 2*(6*m**2 + u)*t**2*u + (8*m
**2 + 3*u)*t*u**2)*u - (t + 3*u - 2*m**2)*t**4)*eps + 3*t**5 + 11*t**4*u + 14*t
**3*u**2 + 6*t**2*u**3 - t*u**4 - u**5)*((t + u)*m**2 + t*u) + 2*(t**5 + 5*t**4*
u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)*t*u)*(2*cf - nc)*c4(-1) + ((2
*((6*m**2*u - t**2 + 2*(m**2 - u)*t)*t**2 + (2*(3*m**2 + u)*t + (2*m**2 + u)*u)*
u**2)*eps + 3*t**4 + 8*t**3*u + 6*t**2*u**2 - u**4)*((t + u)*m**2 + t*u) + 2*(t
**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*t*u)*(2*(ln + 2*lnu) - 5*cf) + (
(2*(4*(m**2 + u)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2 - (t**5 + 3*t**4*u + 2
*t**3*u**2 - 2*t**2*u**3 - 3*t*u**4 - u**5))*eps + 3*t**5 + 11*t**4*u + 14*t**3*
u**2 + 6*t**2*u**3 - t*u**4 - u**5 + 2*(3*t**4 + 8*t**3*u + 6*t**2*u**2 - u**4)*
m**2)*((t + u)*m**2 + t*u) + 2*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 
5*t*u**4 + u**5 + 2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2)*t*u)
*(2*cf - nc)*c6(-1))*(t + u + 4*m**2)*c3u(0)*t*u**2 - 18*(7*((2*((2*t - u + 2*m
**2)*u**4 + (t - 5*u + 2*m**2)*t**4 + 2*(4*t - 5*u + 4*m**2)*t**3*u + 2*(6*t - 5
*u + 6*m**2)*t**2*u**2 + (8*t - 5*u + 8*m**2)*t*u**3)*eps + 5*t**5 + 21*t**4*u +
 34*t**3*u**2 + 26*t**2*u**3 + 9*t*u**4 + u**5)*((t + u)*m**2 + t*u) - 2*(2*t**6
 + 11*t**5*u + 25*t**4*u**2 + 30*t**3*u**3 + 20*t**2*u**4 + 7*t*u**5 + u**6)*t)*
(2*cf - nc)*c4(-1) - (((2*((6*(t - u + m**2)*u + (t - 4*u + 2*m**2)*t)*t**2 + (6
*t**2 - 2*t*u - u**2 + 2*(3*t + u)*m**2)*u**2)*eps + 5*t**4 + 16*t**3*u + 18*t**
2*u**2 + 8*t*u**3 + u**4)*((t + u)*m**2 + t*u) - 2*(2*t**5 + 9*t**4*u + 16*t**3*
u**2 + 14*t**2*u**3 + 6*t*u**4 + u**5)*t)*(35*cf - 38*ln - 4*lnu) - 7*((2*(4*(m
**2 + t)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2 + t**5 + 3*t**4*u + 2*t**3*u**
2 - 2*t**2*u**3 - 3*t*u**4 - u**5)*eps + 5*t**5 + 21*t**4*u + 34*t**3*u**2 + 26*
t**2*u**3 + 9*t*u**4 + u**5 + 2*(5*t**4 + 16*t**3*u + 18*t**2*u**2 + 8*t*u**3 + 
u**4)*m**2)*((t + u)*m**2 + t*u) - 2*(2*t**6 + 11*t**5*u + 25*t**4*u**2 + 30*t**
3*u**3 + 20*t**2*u**4 + 7*t*u**5 + u**6 + 2*(2*t**5 + 9*t**4*u + 16*t**3*u**2 + 
14*t**2*u**3 + 6*t*u**4 + u**5)*m**2)*t)*(2*cf - nc)*c6(-1)))*(t + u + 4*m**2)*
c3(0)*t**2*u + 18*(7*(2*((t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u
**4 + u**5)*eps*m**2 + t**6) - 3*(2*m**2 + t)*(5*t + u)*u**4 + 2*((t + u)*m**2 +
 t*u)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*eps - (3*t - 8*u + 6*m**
2)*t**5 - 3*(5*t - 4*u + 10*m**2)*t**4*u - 2*(15*t - 4*u + 30*m**2)*t**3*u**2 - 
2*(15*t - u + 30*m**2)*t**2*u**3)*(2*cf - nc)*c4(-1) - ((2*((t**4 + 4*t**3*u + 6
*t**2*u**2 + 4*t*u**3 + u**4)*eps*m**2 + t**5) - 3*(2*m**2 + t)*(4*t + u)*u**3 -
 3*(t - 2*u + 2*m**2)*t**4 + 2*((t + u)*m**2 + t*u)*(t**3 + 3*t**2*u + 3*t*u**2 
+ u**3)*eps - 6*(2*t - u + 4*m**2)*t**3*u - 2*(9*t - u + 18*m**2)*t**2*u**2)*(35
*cf - 38*ln - 4*lnu) + 7*((t**5 + 7*t**4*u + 18*t**3*u**2 + 22*t**2*u**3 + 13*t*
u**4 + 3*u**5)*t + 12*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**4 + 2
*(4*t**5 + 21*t**4*u + 42*t**3*u**2 + 40*t**2*u**3 + 18*t*u**4 + 3*u**5)*m**2 - 
2*((4*m**4 + t*u)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4) + 2*(t**5 + 
6*t**4*u + 13*t**3*u**2 + 13*t**2*u**3 + 6*t*u**4 + u**5)*m**2)*eps)*(2*cf - nc)
*c6(-1)))*((t + u)*m**2 + t*u)*(t + u + 4*m**2)*b1(0)*u - 9*(2*(2*(2*(((2*t**6 +
 11*t**5*u + 25*t**4*u**2 + 30*t**3*u**3 + 20*t**2*u**4 + 7*t*u**5 + u**6)*t + 2
*(t**6 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*u**3 + 15*t**2*u**4 + 6*t*u**5 + u**6
)*m**2)*lnu + 3*((t + u)*m**2 + t*u)**2*(7*ln + 2*lnu)*(t**3 + 3*t**2*u + 3*t*u
**2 + u**3)*eps) + (19*(2*t**6 + 11*t**5*u + 25*t**4*u**2 + 30*t**3*u**3 + 20*t
**2*u**4 + 7*t*u**5 + u**6)*t + 2*(t**6 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*u**3
 + 15*t**2*u**4 + 6*t*u**5 + u**6)*m**2)*ln - 30*((t**5 + 3*t**4*u + 4*t**3*u**2
 + 4*t**2*u**3 + 3*t*u**4 + u**5 - 2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 +
 u**4)*m**2)*eps - (t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u
**5))*((t + u)*m**2 + t*u)*cf**2) - (2*((59*t**5 + 219*t**4*u + 328*t**3*u**2 + 
260*t**2*u**3 + 117*t*u**4 + 25*u**5 - 28*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u
**3 + u**4)*m**2*nc + 14*(t**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4
 + u**5)*nc)*ln + 2*(5*t**5 + 21*t**4*u + 40*t**3*u**2 + 44*t**2*u**3 + 27*t*u**
4 + 7*u**5 - 4*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2*nc + 2*(t
**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5)*nc)*lnu)*eps - (4*
(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)*nc - 3*(t**5 +
 t**4*u - 6*t**3*u**2 - 14*t**2*u**3 - 11*t*u**4 - 3*u**5))*(7*ln + 2*lnu))*((t 
+ u)*m**2 + t*u)) + ((2*(5*(23*t**5 + 87*t**4*u + 136*t**3*u**2 + 116*t**2*u**3 
+ 57*t*u**4 + 13*u**5 - 12*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**
2*nc + 6*(t**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5)*nc) + 8
*(t**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5 - 2*(t**4 + 4*t
**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2)*(7*ln + 2*lnu))*eps - (4*(8*lnu + 
15*nc + 28*ln)*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)
 - 45*(t**5 + t**4*u - 6*t**3*u**2 - 14*t**2*u**3 - 11*t*u**4 - 3*u**5)))*((t + 
u)*m**2 + t*u) - 10*(7*(2*t**6 + 11*t**5*u + 25*t**4*u**2 + 30*t**3*u**3 + 20*t
**2*u**4 + 7*t*u**5 + u**6)*t + 2*(t**6 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*u**3
 + 15*t**2*u**4 + 6*t*u**5 + u**6)*m**2 + 18*((t + u)*m**2 + t*u)**2*(t**3 + 3*t
**2*u + 3*t*u**2 + u**3)*eps))*cf + (2*(2*(7*(2*t**7 + 13*t**6*u + 36*t**5*u**2 
+ 55*t**4*u**3 + 50*t**3*u**4 + 27*t**2*u**5 + 8*t*u**6 + u**7)*t + 2*(t**7 + 7*
t**6*u + 21*t**5*u**2 + 35*t**4*u**3 + 35*t**3*u**4 + 21*t**2*u**5 + 7*t*u**6 + 
u**7)*m**2 + 18*((t + u)*m**2 + t*u)**2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**
3 + u**4)*eps + 12*((t**6 + 4*t**5*u + 7*t**4*u**2 + 8*t**3*u**3 + 7*t**2*u**4 +
 4*t*u**5 + u**6 - 2*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 +
 u**5)*m**2)*eps - (t**6 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*u**3 + 15*t**2*u**4
 + 6*t*u**5 + u**6))*((t + u)*m**2 + t*u)*cf) - (2*(23*t**6 + 110*t**5*u + 223*t
**4*u**2 + 252*t**3*u**3 + 173*t**2*u**4 + 70*t*u**5 + 13*u**6 - 24*(t**5 + 5*t
**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)*m**2*nc + 12*(t**6 + 4*t
**5*u + 7*t**4*u**2 + 8*t**3*u**3 + 7*t**2*u**4 + 4*t*u**5 + u**6)*nc)*eps - 3*(
8*(t**6 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*u**3 + 15*t**2*u**4 + 6*t*u**5 + u**
6)*nc - 3*(t**6 + 2*t**5*u - 5*t**4*u**2 - 20*t**3*u**3 - 25*t**2*u**4 - 14*t*u
**5 - 3*u**6)))*((t + u)*m**2 + t*u))*cf + ((2*(23*t**6 + 110*t**5*u + 223*t**4*
u**2 + 252*t**3*u**3 + 173*t**2*u**4 + 70*t*u**5 + 13*u**6 - 12*(t**5 + 5*t**4*u
 + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)*m**2*nc + 6*(t**6 + 4*t**5*u +
 7*t**4*u**2 + 8*t**3*u**3 + 7*t**2*u**4 + 4*t*u**5 + u**6)*nc)*eps - 3*(4*(t**6
 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*u**3 + 15*t**2*u**4 + 6*t*u**5 + u**6)*nc -
 3*(t**6 + 2*t**5*u - 5*t**4*u**2 - 20*t**3*u**3 - 25*t**2*u**4 - 14*t*u**5 - 3*
u**6)))*((t + u)*m**2 + t*u) - 2*(7*(2*t**7 + 13*t**6*u + 36*t**5*u**2 + 55*t**4
*u**3 + 50*t**3*u**4 + 27*t**2*u**5 + 8*t*u**6 + u**7)*t + 2*(t**7 + 7*t**6*u + 
21*t**5*u**2 + 35*t**4*u**3 + 35*t**3*u**4 + 21*t**2*u**5 + 7*t*u**6 + u**7)*m**
2 + 18*((t + u)*m**2 + t*u)**2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)
*eps))*nc)*c4(-1) + (2*(2*(7*(2*t**7 + 13*t**6*u + 36*t**5*u**2 + 55*t**4*u**3 +
 50*t**3*u**4 + 27*t**2*u**5 + 8*t*u**6 + u**7)*t + 4*(t**6 + 6*t**5*u + 15*t**4
*u**2 + 20*t**3*u**3 + 15*t**2*u**4 + 6*t*u**5 + u**6)*m**4 + 2*(15*t**7 + 84*t
**6*u + 196*t**5*u**2 + 245*t**4*u**3 + 175*t**3*u**4 + 70*t**2*u**5 + 14*t*u**6
 + u**7)*m**2 + 18*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4 + 2*(t**3 + 
3*t**2*u + 3*t*u**2 + u**3)*m**2)*((t + u)*m**2 + t*u)**2*eps - 12*((4*((t**4 + 
4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2 + (t**3 + 3*t**2*u + 3*t*u**2 + u
**3)*t*u)*m**2 - (t**6 + 4*t**5*u + 7*t**4*u**2 + 8*t**3*u**3 + 7*t**2*u**4 + 4*
t*u**5 + u**6))*eps + t**6 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*u**3 + 15*t**2*u
**4 + 6*t*u**5 + u**6 + 2*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u
**4 + u**5)*m**2)*((t + u)*m**2 + t*u)*cf) - (2*(2*(23*t**5 + 87*t**4*u + 136*t
**3*u**2 + 116*t**2*u**3 + 57*t*u**4 + 13*u**5 - 24*(t**3 + 3*t**2*u + 3*t*u**2 
+ u**3)*nc*t*u - 24*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2*nc)*m
**2 + 23*t**6 + 110*t**5*u + 223*t**4*u**2 + 252*t**3*u**3 + 173*t**2*u**4 + 70*
t*u**5 + 13*u**6 + 12*(t**6 + 4*t**5*u + 7*t**4*u**2 + 8*t**3*u**3 + 7*t**2*u**4
 + 4*t*u**5 + u**6)*nc)*eps - 3*(8*(t**6 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*u**
3 + 15*t**2*u**4 + 6*t*u**5 + u**6)*nc - 3*(t**6 + 2*t**5*u - 5*t**4*u**2 - 20*t
**3*u**3 - 25*t**2*u**4 - 14*t*u**5 - 3*u**6) + 2*(8*(t**5 + 5*t**4*u + 10*t**3*
u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)*nc - 3*(t**5 + t**4*u - 6*t**3*u**2 - 14*
t**2*u**3 - 11*t*u**4 - 3*u**5))*m**2))*((t + u)*m**2 + t*u))*cf + ((2*(2*(23*t
**5 + 87*t**4*u + 136*t**3*u**2 + 116*t**2*u**3 + 57*t*u**4 + 13*u**5 - 12*(t**3
 + 3*t**2*u + 3*t*u**2 + u**3)*nc*t*u - 12*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*
u**3 + u**4)*m**2*nc)*m**2 + 23*t**6 + 110*t**5*u + 223*t**4*u**2 + 252*t**3*u**
3 + 173*t**2*u**4 + 70*t*u**5 + 13*u**6 + 6*(t**6 + 4*t**5*u + 7*t**4*u**2 + 8*t
**3*u**3 + 7*t**2*u**4 + 4*t*u**5 + u**6)*nc)*eps - 3*(4*(t**6 + 6*t**5*u + 15*t
**4*u**2 + 20*t**3*u**3 + 15*t**2*u**4 + 6*t*u**5 + u**6)*nc - 3*(t**6 + 2*t**5*
u - 5*t**4*u**2 - 20*t**3*u**3 - 25*t**2*u**4 - 14*t*u**5 - 3*u**6) + 2*(4*(t**5
 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)*nc - 3*(t**5 + t**4
*u - 6*t**3*u**2 - 14*t**2*u**3 - 11*t*u**4 - 3*u**5))*m**2))*((t + u)*m**2 + t*
u) - 2*(7*(2*t**7 + 13*t**6*u + 36*t**5*u**2 + 55*t**4*u**3 + 50*t**3*u**4 + 27*
t**2*u**5 + 8*t*u**6 + u**7)*t + 4*(t**6 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*u**
3 + 15*t**2*u**4 + 6*t*u**5 + u**6)*m**4 + 2*(15*t**7 + 84*t**6*u + 196*t**5*u**
2 + 245*t**4*u**3 + 175*t**3*u**4 + 70*t**2*u**5 + 14*t*u**6 + u**7)*m**2 + 18*(
t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4 + 2*(t**3 + 3*t**2*u + 3*t*u**2 
+ u**3)*m**2)*((t + u)*m**2 + t*u)**2*eps))*nc)*c6(-1))*(t + u + 4*m**2)*c4(0)*t
*u - 36*(((2*m**2 + u)*t**5 - 2*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 +
 5*t*u**4 + u**5)*eps*m**2 + (2*m**2 + 3*u)*u**5 + (10*m**2 + 7*u)*t**4*u + 2*(
10*m**2 + 9*u)*t**3*u**2 + 2*(10*m**2 + 11*u)*t**2*u**3 + (10*m**2 + 13*u)*t*u**
4 - 2*((t + u)*m**2 + t*u)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*eps
)*(2*cf - nc)*c4(-1) + ((2*m**2 + 3*u)*u**4 - 2*(t**4 + 4*t**3*u + 6*t**2*u**2 +
 4*t*u**3 + u**4)*eps*m**2 + 2*(4*m**2 + 5*u)*t*u**3 - 2*((t + u)*m**2 + t*u)*(t
**3 + 3*t**2*u + 3*t*u**2 + u**3)*eps + ((2*m**2 + u)*t**2 + 12*(m**2 + u)*u**2 
+ 2*(4*m**2 + 3*u)*t*u)*t**2)*(2*(ln + 2*lnu) - 5*cf) + (2*(t**5 + 6*t**4*u + 16
*t**3*u**2 + 22*t**2*u**3 + 15*t*u**4 + 4*u**5 + 2*(t**4 + 4*t**3*u + 6*t**2*u**
2 + 4*t*u**3 + u**4)*m**2)*m**2 + (t**5 + 7*t**4*u + 18*t**3*u**2 + 22*t**2*u**3
 + 13*t*u**4 + 3*u**5)*u - 2*((4*m**4 + t*u)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*
t*u**3 + u**4) + 2*(t**5 + 6*t**4*u + 13*t**3*u**2 + 13*t**2*u**3 + 6*t*u**4 + u
**5)*m**2)*eps)*(2*cf - nc)*c6(-1))*((t + u)*m**2 + t*u)*(t + u + 4*m**2)*b1u(0)
*t - 18*(2*((4*m**2 + 9*u)*u**5 + 4*(m**2 + 11*u)*t**5 + 5*(4*m**2 + 23*u)*t**4*
u - 4*(5*m**2 - u)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2 + 4*(5
*m**2 + 13*u)*t*u**4 + 5*(8*m**2 + 25*u)*t**2*u**3 - 2*(14*m**2*t**5 + 42*m**2*t
**4*u + 46*m**2*t**3*u**2 + 26*m**2*t**2*u**3 + 12*m**2*t*u**4 + 4*m**2*u**5 + 7
*t**6 + 28*t**5*u + 44*t**4*u**2 + 36*t**3*u**3 + 19*t**2*u**4 + 8*t*u**5 + 2*u
**6)*eps + (40*(m**2 + 4*u)*u**2 + 7*t**3)*t**3)*((t + u)*m**2 + t*u) + 2*((5*t
**6 + 34*t**5*u + 95*t**4*u**2 + 140*t**3*u**3 + 115*t**2*u**4 + 50*t*u**5 + 9*u
**6)*m**4 + 7*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)*
t**3) + (33*t**7 + 151*t**6*u + 297*t**5*u**2 + 347*t**4*u**3 + 283*t**3*u**4 + 
165*t**2*u**5 + 59*t*u**6 + 9*u**7)*m**2)*(t + u + 4*m**2)*(2*cf - nc)*c1(0)*c6(
-1)*t*u)*(t + u + 4*m**2)*(t + u) + 3*(3*((2*(((3*(((3*nc - 2)*nc + 12*cf**2 - 4
*(3*nc - 1)*cf)*((t**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5 
- 2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2)*eps - (t**5 + 5*t**4
*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5))*(t + u + 4*m**2)*c4(-1) - 8
*((nc - 3)*nc + 4*cf**2 - 2*(2*nc - 3)*cf)*((t + u)*m**2 + t*u)*(t + u)**2*eps2*
m**2 + (2*(6*nc - 11 - 6*cf)*cf - (3*nc**2 - 11*nc + 6))*((t**4 + 2*t**3*u + 2*t
**2*u**2 + 2*t*u**3 + u**4 - 2*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2)*eps2 - 
(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*eps)*(t + u + 4*m**2)) - 8*(2*
((7*ln + 2*lnu)*nc + 15*cf**2) - (8*lnu + 15*nc + 28*ln)*cf)*((t + u)*m**2 + t*u
)*(t + u)**2*eps*m**2)*(t + u + 4*m**2)*b2(0) + 48*((15*cf - 14*ln - 4*lnu)*(t +
 u) - 3*(2*cf - nc)*(t**2 + 2*t*u + u**2)*c4(-1) - 3*(t**2 + 2*t*u + u**2 + 2*(t
 + u)*m**2)*(2*cf - nc)*c6(-1))*((t + u)*m**2 + t*u)*(t + u)**2*c1(0)*eps*m**4*
nc)*((t + u)*m**2 + t*u) + (4*((t + u)*m**2 + t*u)**2*(t**3 + 3*t**2*u + 3*t*u**
2 + u**3)*eps2 + (2*eps*m**2 + 3*u)*(t**6 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*u
**3 + 15*t**2*u**4 + 6*t*u**5 + u**6) - (2*(t**5 + 5*t**4*u + 12*t**3*u**2 + 16*
t**2*u**3 + 11*t*u**4 + 3*u**5)*eps2 + (t**5 + t**4*u - 6*t**3*u**2 - 14*t**2*u
**3 - 11*t*u**4 - 3*u**5)*eps)*((t + u)*m**2 + t*u))*(nc - 3 - 2*cf)*(t + u + 4*
m**2)**2*d2u(0)*u + (2*(2*((t + u)*m**2 + t*u)**2*(t**3 + 3*t**2*u + 3*t*u**2 + 
u**3)*eps + (t**6 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*u**3 + 15*t**2*u**4 + 6*t*
u**5 + u**6)*m**2) - (2*(t**5 + 5*t**4*u + 12*t**3*u**2 + 16*t**2*u**3 + 11*t*u
**4 + 3*u**5)*eps + t**5 + t**4*u - 6*t**3*u**2 - 14*t**2*u**3 - 11*t*u**4 - 3*u
**5)*((t + u)*m**2 + t*u))*(2*(ln + 2*lnu) - 5*cf)*(t + u + 4*m**2)**2*d2u(0)*u 
+ (2*(2*((t + u)*m**2 + t*u)**2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4
)*eps + (t**7 + 7*t**6*u + 21*t**5*u**2 + 35*t**4*u**3 + 35*t**3*u**4 + 21*t**2*
u**5 + 7*t*u**6 + u**7)*m**2) - (2*(t**6 + 6*t**5*u + 17*t**4*u**2 + 28*t**3*u**
3 + 27*t**2*u**4 + 14*t*u**5 + 3*u**6)*eps + t**6 + 2*t**5*u - 5*t**4*u**2 - 20*
t**3*u**3 - 25*t**2*u**4 - 14*t*u**5 - 3*u**6)*((t + u)*m**2 + t*u))*(t + u + 4*
m**2)**2*(2*cf - nc)*c4(-1)*d2u(0)*u - 8*(3*(t**2 + 2*t*u + u**2 - 8*(t + u)*m**
2)*(2*cf - nc)*c4(-1) - (t + u - 8*m**2)*(15*cf - 14*ln - 4*lnu) - 3*(2*(3*(t + 
u) + 8*m**2)*m**2 - (t**2 + 2*t*u + u**2))*(2*cf - nc)*c6(-1))*((t + u)*m**2 + t
*u)**2*(t + u)**2*b5(0)*eps*m**2*nc - 6*((4*((t**3 + 3*t**2*u + 3*t*u**2 + u**3)
*m**2 + (t**2 + 2*t*u + u**2)*t*u)*m**2 - (t**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**
2*u**3 + 3*t*u**4 + u**5))*eps2 + (t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3
 + 5*t*u**4 + u**5 + 2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2)*
eps)*((nc - 3)*nc + 4*cf**2 - 2*(2*nc - 3)*cf)*((t + u)*m**2 + t*u)*(t + u + 4*m
**2)**2*c6(0) + 6*((4*((t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2 + 
(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*t*u)*m**2 - (t**6 + 4*t**5*u + 7*t**4*u**2 +
 8*t**3*u**3 + 7*t**2*u**4 + 4*t*u**5 + u**6))*eps + t**6 + 6*t**5*u + 15*t**4*u
**2 + 20*t**3*u**3 + 15*t**2*u**4 + 6*t*u**5 + u**6 + 2*(t**5 + 5*t**4*u + 10*t
**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)*m**2)*((t + u)*m**2 + t*u)*(t + u + 4
*m**2)**2*(4*cf**2 - 4*cf*nc + nc**2)*c4(-1)*c6(0) - ((3*(t**5 + 3*t**4*u + 4*t
**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5 - 2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*
t*u**3 + u**4)*m**2)*nc + 2*(2*t + 7*u + 18*m**2)*(t**4 + 4*t**3*u + 6*t**2*u**2
 + 4*t*u**3 + u**4))*eps + (7*t - 11*u - 8*m**2)*(t**4 + 4*t**3*u + 6*t**2*u**2 
+ 4*t*u**3 + u**4) - 3*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4
 + u**5)*nc)*((t + u)*m**2 + t*u)*(t + u + 4*m**2)*(2*cf - nc)*(t + u)*b5(0)*c4(
-1)) - 7*((2*(3*t**5 + 11*t**4*u + 16*t**3*u**2 + 12*t**2*u**3 + 5*t*u**4 + u**5
)*eps2 + (t**5 + t**4*u - 6*t**3*u**2 - 14*t**2*u**3 - 11*t*u**4 - 3*u**5)*eps -
 4*((t + u)*m**2 + t*u)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*eps2)*((t + u)*m**2 
+ t*u) - (2*(2*t**6 + 11*t**5*u + 25*t**4*u**2 + 30*t**3*u**3 + 20*t**2*u**4 + 7
*t*u**5 + u**6)*eps - 3*(t**6 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*u**3 + 15*t**2
*u**4 + 6*t*u**5 + u**6))*t)*(nc - 3 - 2*cf)*(t + u + 4*m**2)**2*d2(0)*t + ((2*(
3*t**5 + 11*t**4*u + 16*t**3*u**2 + 12*t**2*u**3 + 5*t*u**4 + u**5)*eps + t**5 +
 t**4*u - 6*t**3*u**2 - 14*t**2*u**3 - 11*t*u**4 - 3*u**5 - 4*((t + u)*m**2 + t*
u)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*eps)*((t + u)*m**2 + t*u) - 2*(2*t**6 + 
11*t**5*u + 25*t**4*u**2 + 30*t**3*u**3 + 20*t**2*u**4 + 7*t*u**5 + u**6)*t)*(t 
+ u + 4*m**2)**2*(35*cf - 38*ln - 4*lnu)*d2(0)*t - (4*(2*(7*t**5 + 26*t**4*u + 
34*t**3*u**2 + 16*t**2*u**3 - t*u**4 - 2*u**5) - 3*(t**5 + 5*t**4*u + 10*t**3*u
**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)*nc)*m**2 + 5*(t**6 + 6*t**5*u + 15*t**4*u
**2 + 20*t**3*u**3 + 15*t**2*u**4 + 6*t*u**5 + u**6) + 2*(5*(t**5 + 5*t**4*u + 
10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)*(t - u) + 6*(t**5 + 3*t**4*u + 4*
t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5)*m**2*nc - 4*(3*(t**4 + 4*t**3*u + 6*t
**2*u**2 + 4*t*u**3 + u**4)*nc + 10*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*(t - u))
*m**4)*eps)*((t + u)*m**2 + t*u)*(t + u + 4*m**2)*(2*cf - nc)*(t + u)*c1(0)*c4(
-1) - 7*((2*(3*t**6 + 14*t**5*u + 27*t**4*u**2 + 28*t**3*u**3 + 17*t**2*u**4 + 6
*t*u**5 + u**6)*eps + t**6 + 2*t**5*u - 5*t**4*u**2 - 20*t**3*u**3 - 25*t**2*u**
4 - 14*t*u**5 - 3*u**6 - 4*((t + u)*m**2 + t*u)*(t**4 + 4*t**3*u + 6*t**2*u**2 +
 4*t*u**3 + u**4)*eps)*((t + u)*m**2 + t*u) - 2*(2*t**7 + 13*t**6*u + 36*t**5*u
**2 + 55*t**4*u**3 + 50*t**3*u**4 + 27*t**2*u**5 + 8*t*u**6 + u**7)*t)*(t + u + 
4*m**2)**2*(2*cf - nc)*c4(-1)*d2(0)*t - (2*((5*t**6 + 34*t**5*u + 95*t**4*u**2 +
 140*t**3*u**3 + 115*t**2*u**4 + 50*t*u**5 + 9*u**6)*m**2 + 14*(t**4 + 4*t**3*u 
+ 6*t**2*u**2 + 4*t*u**3 + u**4)*t**3)*eps - 3*(7*t - 2*u + 10*m**2)*(t**6 + 6*t
**5*u + 15*t**4*u**2 + 20*t**3*u**3 + 15*t**2*u**4 + 6*t*u**5 + u**6) + 4*((7*t
**5 + 37*t**4*u + 78*t**3*u**2 + 82*t**2*u**3 + 43*t*u**4 + 9*u**5 - 10*(t**4 + 
4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2)*eps - 2*(7*t**5 + 21*t**4*u + 23
*t**3*u**2 + 13*t**2*u**3 + 6*t*u**4 + 2*u**5)*eps2)*((t + u)*m**2 + t*u))*(nc -
 3 - 2*cf)*(t + u + 4*m**2)**2*c1(0) - 2*(2*(7*t**6 + 44*t**5*u + 115*t**4*u**2 
+ 160*t**3*u**3 + 125*t**2*u**4 + 52*t*u**5 + 9*u**6 - 10*(t**5 + 5*t**4*u + 10*
t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)*m**2 - 2*(7*t**6 + 28*t**5*u + 44*t
**4*u**2 + 36*t**3*u**3 + 19*t**2*u**4 + 8*t*u**5 + 2*u**6)*eps)*((t + u)*m**2 +
 t*u) + (5*t**7 + 39*t**6*u + 129*t**5*u**2 + 235*t**4*u**3 + 255*t**3*u**4 + 
165*t**2*u**5 + 59*t*u**6 + 9*u**7)*m**2 + 14*(t**5 + 5*t**4*u + 10*t**3*u**2 + 
10*t**2*u**3 + 5*t*u**4 + u**5)*t**3)*(t + u + 4*m**2)**2*(2*cf - nc)*c1(0)*c4(
-1) + 2*(2*((t**7 + 7*t**6*u + 21*t**5*u**2 + 35*t**4*u**3 + 35*t**3*u**4 + 21*t
**2*u**5 + 7*t*u**6 + u**7 + 2*(t**6 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*u**3 + 
15*t**2*u**4 + 6*t*u**5 + u**6)*m**2)*m**2 + 2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 
4*t*u**3 + u**4 + 2*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2)*((t + u)*m**2 + t*
u)**2*eps) - (2*(t**6 + 6*t**5*u + 17*t**4*u**2 + 28*t**3*u**3 + 27*t**2*u**4 + 
14*t*u**5 + 3*u**6 + 2*(t**5 + 5*t**4*u + 12*t**3*u**2 + 16*t**2*u**3 + 11*t*u**
4 + 3*u**5)*m**2)*eps + t**6 + 2*t**5*u - 5*t**4*u**2 - 20*t**3*u**3 - 25*t**2*u
**4 - 14*t*u**5 - 3*u**6 + 2*(t**5 + t**4*u - 6*t**3*u**2 - 14*t**2*u**3 - 11*t*
u**4 - 3*u**5)*m**2)*((t + u)*m**2 + t*u))*(t + u + 4*m**2)**2*(2*cf - nc)*c6(-1
)*d2u(0)*u)*(t + u) - 2*(3*((3*nc - 2)*nc + 12*cf**2 - 4*(3*nc - 1)*cf)*(t + u)*
b2(0) - 2*((t + u + 4*m**2)*b2(0) - 3*(t + u)*log(m**2/mur**2)*beta0)*(2*cf - nc
))*((4*((t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2 + (t**2 + 2*t*u + u**2)*t*u)*m
**2 - (t**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5))*eps + t**
5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5 + 2*(t**4 + 4*t**3*
u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2)*((t + u)*m**2 + t*u)*(t + u + 4*m**2)**
2*c6(-1) + 7*((2*(4*((t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2 - (t
**4 + 2*t**3*u - 2*t*u**3 - u**4)*t)*m**2 - (3*t**6 + 12*t**5*u + 19*t**4*u**2 +
 16*t**3*u**3 + 9*t**2*u**4 + 4*t*u**5 + u**6))*eps - (t**6 + 2*t**5*u - 5*t**4*
u**2 - 20*t**3*u**3 - 25*t**2*u**4 - 14*t*u**5 - 3*u**6 + 2*(t**5 + t**4*u - 6*t
**3*u**2 - 14*t**2*u**3 - 11*t*u**4 - 3*u**5)*m**2))*((t + u)*m**2 + t*u) + 2*(2
*t**7 + 13*t**6*u + 36*t**5*u**2 + 55*t**4*u**3 + 50*t**3*u**4 + 27*t**2*u**5 + 
8*t*u**6 + u**7 + 2*(2*t**6 + 11*t**5*u + 25*t**4*u**2 + 30*t**3*u**3 + 20*t**2*
u**4 + 7*t*u**5 + u**6)*m**2)*t)*(t + u + 4*m**2)**2*(2*cf - nc)*(t + u)*c6(-1)*
d2(0)*t) + 2*(72*((8*(15*cf - 14*ln - 4*lnu - 3*(2*cf - nc)*(t + u)*c4(-1) - 3*(
t + u + 2*m**2)*(2*cf - nc)*c6(-1))*eps*m**2 - (6*((t + u)*c1(0) + 4)*m**2 + (t 
+ u - 8*m**2)*b5(0))*(nc - 3 - 2*cf)*eps2)*(t + u)*nc + ((t**2 + 2*t*u + u**2 + 
2*(t + u)*m**2)*c6(-1) + (t**2 + 2*t*u + u**2)*c4(-1))*(t + u + 4*m**2)*(4*cf**2
 - 4*cf*nc + nc**2)*b2(0)*eps)*((t + u)*m**2 + t*u)*(t + u)**2*m**2 - (6*(((t**5
 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5 - 2*(t**4 + 4*t**3*u +
 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2)*eps - (t**5 + 5*t**4*u + 10*t**3*u**2 + 10
*t**2*u**3 + 5*t*u**4 + u**5))*(2*cf - nc)*c4(-1) + ((t**4 + 2*t**3*u + 2*t**2*u
**2 + 2*t*u**3 + u**4 - 2*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2)*eps2 - (t**4
 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*eps)*(nc - 3 - 2*cf))*((t + u + 4*m
**2)*b2(0) - 3*(t + u)*log(m**2/mur**2)*beta0) - (2*((t + u + 4*m**2)*b2(0) - 3*
(t + u)*log(m**2/mur**2)*beta0)*(15*cf - 14*ln - 4*lnu) - 3*(90*cf**2 - 84*cf*ln
 - 24*cf*lnu - 45*cf*nc + 30*cf + 42*ln*nc - 28*ln + 12*lnu*nc - 8*lnu)*(t + u)*
b2(0))*((t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4 - 2*(t**3 + 3*t**2*u + 
3*t*u**2 + u**3)*m**2)*eps - (t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)))
*(t + u + 4*m**2)**2)*((t + u)*m**2 + t*u))*t*u)*(t**2 + 2*t*u + u**2) - ((3*(((
3*(((4*((t + u)*m**2 + t*u)*(10*eps*m**2 + 7*eps*t - 20*m**2 - 14*t + 4*u)*(t**4
 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4) + 118*m**2*t**6 + 668*m**2*t**5*u +
 1570*m**2*t**4*u**2 + 1960*m**2*t**3*u**3 + 1370*m**2*t**2*u**4 + 508*m**2*t*u
**5 + 78*m**2*u**6 + 77*t**7 + 416*t**6*u + 915*t**5*u**2 + 1030*t**4*u**3 + 595
*t**3*u**4 + 132*t**2*u**5 - 19*t*u**6 - 10*u**7 - 2*(7*(2*m**2 + t)*(2*t**6 + 
11*t**5*u + 25*t**4*u**2 + 30*t**3*u**3 + 20*t**2*u**4 + 7*t*u**5 + u**6) - 2*(t
**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)*(t - u)*m**2)*
eps)*(nc - 3 - 2*cf)*c1(0) - 6*(2*(6*nc - 11 - 6*cf)*cf - (3*nc**2 - 11*nc + 6))
*((t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4 - 2*(t**3 + 3*t**2*u + 3*t*u
**2 + u**3)*m**2)*eps - (t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4))*((t +
 u)*m**2 + t*u)*b2(1) - 2*(2*(2*((t + u)*m**2 + t*u)**2*(t**3 + 3*t**2*u + 3*t*u
**2 + u**3)*eps + (t**6 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*u**3 + 15*t**2*u**4 
+ 6*t*u**5 + u**6)*m**2) - (2*(t**5 + 5*t**4*u + 12*t**3*u**2 + 16*t**2*u**3 + 
11*t*u**4 + 3*u**5)*eps + t**5 + t**4*u - 6*t**3*u**2 - 14*t**2*u**3 - 11*t*u**4
 - 3*u**5)*((t + u)*m**2 + t*u))*(nc - 3 - 2*cf)*d2u(1)*u + 12*((4*((t**3 + 3*t
**2*u + 3*t*u**2 + u**3)*m**2 + (t**2 + 2*t*u + u**2)*t*u)*m**2 - (t**5 + 3*t**4
*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5))*eps + t**5 + 5*t**4*u + 10*t
**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5 + 2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4
*t*u**3 + u**4)*m**2)*((nc - 3)*nc + 4*cf**2 - 2*(2*nc - 3)*cf)*((t + u)*m**2 + 
t*u)*c6(1))*(t + u + 4*m**2) + 12*(((t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + 
u**4 - 2*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2)*eps - (t**4 + 4*t**3*u + 6*t
**2*u**2 + 4*t*u**3 + u**4))*(t + u + 4*m**2)*b2(0) + 4*((t + u)*m**2 + t*u)*(b2
(1) + 2*b2(0))*(t + u)**2*eps*m**2)*((nc - 3)*nc + 4*cf**2 - 2*(2*nc - 3)*cf)*((
t + u)*m**2 + t*u) + 7*((2*(3*t**5 + 11*t**4*u + 16*t**3*u**2 + 12*t**2*u**3 + 5
*t*u**4 + u**5)*eps + t**5 + t**4*u - 6*t**3*u**2 - 14*t**2*u**3 - 11*t*u**4 - 3
*u**5 - 4*((t + u)*m**2 + t*u)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*eps)*((t + u)
*m**2 + t*u) - 2*(2*t**6 + 11*t**5*u + 25*t**4*u**2 + 30*t**3*u**3 + 20*t**2*u**
4 + 7*t*u**5 + u**6)*t)*(nc - 3 - 2*cf)*(t + u + 4*m**2)*d2(1)*t) - 8*((2*nlf - 
27 + 19*nc - 18*cf)*cf - (5*nc**2 - 3*nlf + (nlf - 15)*nc))*((t**4 + 2*t**3*u + 
2*t**2*u**2 + 2*t*u**3 + u**4 - 2*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2)*eps 
- (t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4))*((t + u)*m**2 + t*u)*(t + u
 + 4*m**2)*b5(0) + 12*(((4*nlf + 27 - 19*nc)*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*
t*u**3 + u**4 - 2*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2)*eps - (4*nlf + 11 - 
19*nc)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4) + 18*((t**4 + 2*t**3*u 
+ 2*t**2*u**2 + 2*t*u**3 + u**4 - 2*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2)*
eps - (t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4))*cf)*cf - ((6*(nlf - 4) 
+ 5*nc**2 - (2*nlf + 7)*nc)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4) - 
(5*nc**2 + 6*nlf - (2*nlf + 15)*nc)*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + 
u**4 - 2*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2)*eps))*((t + u)*m**2 + t*u)*(t
 + u + 4*m**2)*b5(1))*u + 12*((2*m**2 + 3*u)*u**4 - 2*(t**4 + 4*t**3*u + 6*t**2*
u**2 + 4*t*u**3 + u**4)*eps*m**2 + 2*(4*m**2 + 5*u)*t*u**3 - 2*((t + u)*m**2 + t
*u)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*eps + ((2*m**2 + u)*t**2 + 12*(m**2 + u)
*u**2 + 2*(4*m**2 + 3*u)*t*u)*t**2)*(nc - 3 - 2*cf)*((t + u)*m**2 + t*u)*(t + u 
+ 4*m**2)*b1u(1) + 12*((2*((6*m**2*u - t**2 + 2*(m**2 - u)*t)*t**2 + (2*(3*m**2 
+ u)*t + (2*m**2 + u)*u)*u**2)*eps + 3*t**4 + 8*t**3*u + 6*t**2*u**2 - u**4)*((t
 + u)*m**2 + t*u) + 2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*t*u)*(nc
 - 3 - 2*cf)*(t + u + 4*m**2)*c3u(1)*u**2 + 42*((2*((6*(t - u + m**2)*u + (t - 4
*u + 2*m**2)*t)*t**2 + (6*t**2 - 2*t*u - u**2 + 2*(3*t + u)*m**2)*u**2)*eps + 5*
t**4 + 16*t**3*u + 18*t**2*u**2 + 8*t*u**3 + u**4)*((t + u)*m**2 + t*u) - 2*(2*t
**5 + 9*t**4*u + 16*t**3*u**2 + 14*t**2*u**3 + 6*t*u**4 + u**5)*t)*(nc - 3 - 2*
cf)*(t + u + 4*m**2)*c3(1)*t*u + 24*((2*(3*((t**3 + 3*t**2*u + 3*t*u**2 + u**3)*
nc**2 + 14*(t**2 + 2*t*u + u**2)*(t - u)) - (23*t**3 + 41*t**2*u + 13*t*u**2 - 5
*u**3)*nc)*m**2 - 3*(nc - 3)*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4)*
nc)*eps + 3*((t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*nc + 12*(t**2 + 2
*t*u + u**2)*(t - u)*m**2 - 4*((t + u)*m**2 + t*u)*(t + u)*eps*m**2*nc)*(nc - 3)
 + 2*(3*(4*(5*nc - 12 - 8*cf)*((t + u)*m**2 + t*u)*(t + u)*eps*m**2 - ((t**4 + 4
*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*nc + 12*(t**2 + 2*t*u + u**2)*(t - u)*m
**2)) - (2*(3*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*nc - 14*(t**2 + 2*t*u + u**2)*
(t - u))*m**2 - 3*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4)*nc)*eps)*cf)
*((t + u)*m**2 + t*u)*(t + u)*u - 3*(4*(3*(2*(7*t**4 + 19*t**3*u + 15*t**2*u**2 
+ t*u**3 - 2*u**4) + (t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*nc**2) - 
(23*t**4 + 74*t**3*u + 84*t**2*u**2 + 38*t*u**3 + 5*u**4)*nc)*m**2 - 5*(nc - 3)*
(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5) + 2*(4*((t**3 
- 17*t**2*u - 37*t*u**2 - 19*u**3)*nc - 30*(t**2 + 2*t*u + u**2)*(t - u) + 3*(t
**3 + 3*t**2*u + 3*t*u**2 + u**3)*nc**2)*m**4 - (5*(t**4 + 4*t**3*u + 6*t**2*u**
2 + 4*t*u**3 + u**4)*(t - u) + 6*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**
4)*m**2*nc)*(nc - 3))*eps + 2*(4*(2*(7*t**4 + 19*t**3*u + 15*t**2*u**2 + t*u**3 
- 2*u**4) - 3*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*nc)*m**2 + 5*(t
**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5) + 2*(5*(t**4 + 4
*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*(t - u) + 6*(t**4 + 2*t**3*u + 2*t**2*u
**2 + 2*t*u**3 + u**4)*m**2*nc - 4*(3*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*nc + 
10*(t**2 + 2*t*u + u**2)*(t - u))*m**4)*eps)*cf)*((t + u)*m**2 + t*u)*(t + u)*c1
(1)*u + 6*((2*(8*t**4 + 23*t**3*u + 21*t**2*u**2 + 5*t*u**3 - u**4 - 4*(t**3 + 3
*t**2*u + 3*t*u**2 + u**3)*m**2) - 3*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 +
 u**4)*nc)*nc - 3*(7*t - 11*u - 8*m**2)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3) - 2*
((3*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4 - 2*(t**3 + 3*t**2*u + 3*t*
u**2 + u**3)*m**2)*nc + 2*(2*t + 7*u + 18*m**2)*(t**3 + 3*t**2*u + 3*t*u**2 + u
**3))*eps + (7*t - 11*u - 8*m**2)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3) - 3*(t**4 
+ 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*nc)*cf - ((((5*t + 4*u - 36*m**2)*t
**2 - 12*(t + 2*u + 9*m**2)*(t + u)*u)*t - (4*t + 5*u + 36*m**2)*u**3)*nc + 3*((
2*(nc - 3)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*m**2 - (t**4 + 2*t**3*u + 2*t**2*
u**2 + 2*t*u**3 + u**4)*nc)*nc + 2*(2*t + 7*u + 18*m**2)*(t**3 + 3*t**2*u + 3*t*
u**2 + u**3)))*eps)*((t + u)*m**2 + t*u)*(t + u)*b5(1)*u)*(t + u + 4*m**2)*(t + 
u) - (3*(2*(7*(11*t**5 + 51*t**4*u + 94*t**3*u**2 + 86*t**2*u**3 + 39*t*u**4 + 7
*u**5 - 2*(2*t**5 + 9*t**4*u + 16*t**3*u**2 + 14*t**2*u**3 + 6*t*u**4 + u**5)*
eps + 4*((t + u)*m**2 + t*u)*(eps - 2)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3))*c3(0
)*t**2 - 2*((9*t**5 + 41*t**4*u + 74*t**3*u**2 + 66*t**2*u**3 + 29*t*u**4 + 5*u
**5 - 2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*eps*t)*u - 2*((t + u)*
m**2 + t*u)*((t - u)*eps + 4*u)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3))*c3u(0)*u - 
((9*t**6 + 50*t**5*u + 115*t**4*u**2 + 140*t**3*u**3 + 95*t**2*u**4 + 34*t*u**5 
+ 5*u**6 - 2*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + u**5)*
eps*t)*u - 2*((t + u)*m**2 + t*u)*((t - u)*eps + 4*u)*(t**4 + 4*t**3*u + 6*t**2*
u**2 + 4*t*u**3 + u**4))*d2u(0)*u) + 7*(11*t**6 + 62*t**5*u + 145*t**4*u**2 + 
180*t**3*u**3 + 125*t**2*u**4 + 46*t*u**5 + 7*u**6 - 2*(2*t**6 + 11*t**5*u + 25*
t**4*u**2 + 30*t**3*u**3 + 20*t**2*u**4 + 7*t*u**5 + u**6)*eps + 4*((t + u)*m**2
 + t*u)*(eps - 2)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4))*d2(0)*t**2 
- (77*t**7 + 416*t**6*u + 915*t**5*u**2 + 1030*t**4*u**3 + 595*t**3*u**4 + 132*t
**2*u**5 - 19*t*u**6 - 10*u**7 - 2*(14*t**6 + 75*t**5*u + 165*t**4*u**2 + 190*t
**3*u**3 + 120*t**2*u**4 + 39*t*u**5 + 5*u**6)*eps*t + 4*((8*t**5 + 31*t**4*u + 
44*t**3*u**2 + 26*t**2*u**3 + 4*t*u**4 - u**5)*eps - 2*(7*t**5 + 26*t**4*u + 34*
t**3*u**2 + 16*t**2*u**3 - t*u**4 - 2*u**5))*((t + u)*m**2 + t*u))*c4(0) - 2*(2*
(7*t**5 + 37*t**4*u + 78*t**3*u**2 + 82*t**2*u**3 + 43*t*u**4 + 9*u**5 - 10*(t**
4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*m**2 - 2*(7*t**5 + 21*t**4*u + 23*
t**3*u**2 + 13*t**2*u**3 + 6*t*u**4 + 2*u**5)*eps)*((t + u)*m**2 + t*u) + (5*t**
6 + 34*t**5*u + 95*t**4*u**2 + 140*t**3*u**3 + 115*t**2*u**4 + 50*t*u**5 + 9*u**
6)*m**2 + 14*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*t**3)*c1(1))*(t +
 u + 4*m**2)**2*(t + u)*u + 2*(12*((6*(2*(t + u - 12*m**2) - (t**2 + 2*t*u + u**
2)*c1(0) + 2*(b5(0) - 3*c1(1)*m**2)*(t + u) - (t + u - 8*m**2)*b5(1))*((t + u)*m
**2 + t*u)*(t + u)*m**2*nc - ((2*m**2 + t)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*
u**3 + u**4)*c1(0) - (t**3 + 3*t**2*u + 3*t*u**2 + u**3)*(t - u)*b5(0))*(t + u +
 4*m**2))*(t + u)*u - (2*((t + u)*m**2 + t*u)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3
) - (t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*u)*(t + u + 4*m**2)**2*b1u
(0))*(t + u)*eps - ((t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4 - 2*(t**3 +
 3*t**2*u + 3*t*u**2 + u**3)*m**2)*eps - (t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u
**3 + u**4))*(2*(t + u + 4*m**2)*(3*b2(1) + 2*b2(0)) - 9*(t + u)*log(m**2/mur**2
)**2*beta0)*(t + u + 4*m**2)**2*u)*((t + u)*m**2 + t*u))*(nc - 3 - 2*cf))*t - (
16*((2*((14*nc**2 - 3*nlf)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*t*u + 3*(9*t**5 +
 98*t**4*u + 303*t**3*u**2 + 411*t**2*u**3 + 260*t*u**4 + 63*u**5) - (9*t**5 + 
140*t**4*u + 429*t**3*u**2 + 537*t**2*u**3 + 302*t*u**4 + 63*u**5 - (t**3 + 3*t
**2*u + 3*t*u**2 + u**3)*nlf*t*u)*nc)*m**2 - ((nlf - 41 + 14*nc)*nc - 3*(nlf + 1
))*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4)*t*u)*eps + ((nlf - 41 + 14*
nc)*nc - 3*(nlf + 1))*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*t*u + 9*
(nc - 3)*(2*t**5 + 29*t**4*u + 96*t**3*u**2 + 134*t**2*u**3 + 86*t*u**4 + 21*u**
5)*m**2 - 2*((nlf + 82 - 13*nc)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4
)*t*u + 9*(2*t**5 + 29*t**4*u + 96*t**3*u**2 + 134*t**2*u**3 + 86*t*u**4 + 21*u
**5)*m**2 - 54*((t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4 - 2*(t**3 + 3*t
**2*u + 3*t*u**2 + u**3)*m**2)*eps - (t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 +
 u**4))*cf*t*u - (2*((13*nc - nlf)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*t*u + 9*t
**5 + 17*t**4*u + 60*t**3*u**2 + 168*t**2*u**3 + 179*t*u**4 + 63*u**5)*m**2 + (
nlf + 82 - 13*nc)*(t**4 + 2*t**3*u + 2*t**2*u**2 + 2*t*u**3 + u**4)*t*u)*eps)*cf
)*((t + u)*m**2 + t*u) - 9*((2*(3*(4*(nc - 3)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4
*t*u**3 + u**4)*m**2*nc + 23*t**5 + 87*t**4*u + 136*t**3*u**2 + 116*t**2*u**3 + 
57*t*u**4 + 13*u**5) - (5*t**5 + 33*t**4*u + 64*t**3*u**2 + 44*t**2*u**3 + 3*t*u
**4 - 5*u**5 + 6*(t**5 + 3*t**4*u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5)
*nc)*nc)*eps + 3*(4*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5*t*u**4 + 
u**5)*nc**2 + 9*(t**5 + t**4*u - 6*t**3*u**2 - 14*t**2*u**3 - 11*t*u**4 - 3*u**5
) - 3*(5*t**5 + 21*t**4*u + 34*t**3*u**2 + 26*t**2*u**3 + 9*t*u**4 + u**5)*nc))*
((t + u)*m**2 + t*u) + 2*(7*(2*t**6 + 11*t**5*u + 25*t**4*u**2 + 30*t**3*u**3 + 
20*t**2*u**4 + 7*t*u**5 + u**6)*t + 2*(t**6 + 6*t**5*u + 15*t**4*u**2 + 20*t**3*
u**3 + 15*t**2*u**4 + 6*t*u**5 + u**6)*m**2 + 18*((t + u)*m**2 + t*u)**2*(t**3 +
 3*t**2*u + 3*t*u**2 + u**3)*eps)*(nc - 3) - 2*(2*(7*(2*t**6 + 11*t**5*u + 25*t
**4*u**2 + 30*t**3*u**3 + 20*t**2*u**4 + 7*t*u**5 + u**6)*t + 2*(t**6 + 6*t**5*u
 + 15*t**4*u**2 + 20*t**3*u**3 + 15*t**2*u**4 + 6*t*u**5 + u**6)*m**2 + 18*((t +
 u)*m**2 + t*u)**2*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*eps + 12*((t**5 + 3*t**4*
u + 4*t**3*u**2 + 4*t**2*u**3 + 3*t*u**4 + u**5 - 2*(t**4 + 4*t**3*u + 6*t**2*u
**2 + 4*t*u**3 + u**4)*m**2)*eps - (t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**
3 + 5*t*u**4 + u**5))*((t + u)*m**2 + t*u)*cf) - (2*(5*t**5 + 33*t**4*u + 64*t**
3*u**2 + 44*t**2*u**3 + 3*t*u**4 - 5*u**5 + 12*(t**5 + 3*t**4*u + 4*t**3*u**2 + 
4*t**2*u**3 + 3*t*u**4 + u**5)*nc - 12*(2*nc - 3)*(t**4 + 4*t**3*u + 6*t**2*u**2
 + 4*t*u**3 + u**4)*m**2)*eps + 3*(3*(5*t**5 + 21*t**4*u + 34*t**3*u**2 + 26*t**
2*u**3 + 9*t*u**4 + u**5) - 8*(t**5 + 5*t**4*u + 10*t**3*u**2 + 10*t**2*u**3 + 5
*t*u**4 + u**5)*nc))*((t + u)*m**2 + t*u))*cf)*c4(1)*t*u + 126*(2*((t**4 + 4*t**
3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*eps*m**2 + t**5) - 3*(2*m**2 + t)*(4*t + u)
*u**3 - 3*(t - 2*u + 2*m**2)*t**4 + 2*((t + u)*m**2 + t*u)*(t**3 + 3*t**2*u + 3*
t*u**2 + u**3)*eps - 6*(2*t - u + 4*m**2)*t**3*u - 2*(9*t - u + 18*m**2)*t**2*u
**2)*(nc - 3 - 2*cf)*((t + u)*m**2 + t*u)*b1(1)*u)*(t + u + 4*m**2)**2*(t + u))*
(t**2 + 2*t*u + u**2) - 18*(((2*(2*((7*ln + 2*lnu)*nc + 15*cf**2) - 3*(4*cf**2 -
 4*cf*nc + nc**2)*(t + u)*c4(-1)) - 3*(t + u + 2*m**2)*(4*cf**2 - 4*cf*nc + nc**
2)*c6(-1) - 2*(8*lnu + 15*nc + 28*ln)*cf)*(t + u + 2*m**2)*c6(-1) + 2*(2*((7*ln 
+ 2*lnu)*nc + 15*cf**2) - (8*lnu + 15*nc + 28*ln)*cf)*(t + u)*c4(-1) - (75*cf**2
 - 140*cf*ln - 40*cf*lnu + 76*ln**2 + 16*ln*lnu + 16*lnu**2 + 3*(4*cf**2 - 4*cf*
nc + nc**2)*(t + u)**2*c4(-1)**2))*((t**2 + u**2 - 2*(t + u)*m**2)*eps2 - (t**2 
+ 2*t*u + u**2)*eps) + 2*((15*(nc - 3) + 8*lnu + 28*ln)*cf - 2*((7*ln + 2*lnu)*(
nc - 3) + 15*cf**2) + 3*((nc - 3)*nc + 4*cf**2 - 2*(2*nc - 3)*cf)*((t + u + 2*m
**2)*c6(-1) + (t + u)*c4(-1)))*((t**2 + u**2 - 2*(t + u)*m**2)*eps3 - (t**2 + 2*
t*u + u**2)*eps2) + 3*(4*(nc - 3 - cf)*cf - (nc**2 - 6*nc + 9))*((t**2 + u**2 - 
2*(t + u)*m**2)*eps4 - (t**2 + 2*t*u + u**2)*eps3))*((t + u)*m**2 + t*u)*(t + u 
+ 4*m**2)**2*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*(t + u)*t*u))*(t 
+ u)**4 + 2*((((((((27*(7*(3*t**2 + u**2 - 2*(t + u)*m**2)*(c4(2) - d2(2)*t) + 2
*(t**2 + 3*u**2 - 2*(t + u)*m**2)*(c4(2) - d2u(2)*u))*(t + u) + 4*(5*(nlf + 1) -
 38*nc)*(t**2 + u**2 - 2*(t + u)*m**2) - 81*(3*nc - 2 - 6*cf)*(t**2 + u**2 - 2*(
t + u)*m**2)*b2(2) - 54*(5*nc - 2*nlf - 9*cf)*(t**2 + u**2 - 2*(t + u)*m**2)*b5(
2))*u - 108*((2*m**2 - u)*(t + u) + 2*t*u)*(t + u)*b1u(1))*((t + u)*m**2 + t*u) 
- 54*((c4(1) - d2u(1)*u)*(t + u) - 2*c3u(1)*u)*((t**2 - u**2)*m**2 + 2*t**2*u)*(
t + u)*u)*(t + u + 4*m**2) - 108*(((t + u)*t - 8*m**4)*c1(1) - (t - u)*b5(1))*((
t + u)*m**2 + t*u)*(t + u)**2*u - 36*(nlf + 1 + 14*nc + 72*cf)*(t**2 + u**2 - 2*
(t + u)*m**2)*((t + u)*m**2 + t*u)*(t + u + 4*m**2)*u - 12*(3*(5*nc + nlf - 9*cf
)*b5(1) + (nc + 2*nlf)*b5(0))*(t**2 + u**2 - 2*(t + u)*m**2)*((t + u)*m**2 + t*u
)*(t + u + 4*m**2)*u - 54*((2*m**2 + u)*(t + u)*c1(0) - 2*c3u(0)*u**2 + (c4(0) -
 d2u(0)*u)*(t + u)*u)*(3*t**2 + u**2 - 4*(t + u)*m**2)*(t + u + 4*m**2)*(t + u)*
u + 189*((c1(1) + 2*c1(0))*(2*m**2 + t)*(t + u) - 2*(c3(1) + 2*c3(0))*t**2 + (c4
(1) + 2*c4(0) - (d2(1) + 2*d2(0))*t)*(t + u)*t)*(2*t**2 + t*u + u**2 - 2*(t + u)
*m**2)*(t + u + 4*m**2)*(t + u)*u + 54*(((t**2 + 2*t*u + u**2 - 8*m**4)*(t - u) 
+ 4*(t + u + 4*m**2)*u**2)*c1(2) + 2*(t + u + 4*m**2)*(t - u - 2*m**2)*c3u(2)*u)
*((t + u)*m**2 + t*u)*(t + u)*u - 189*(((t**2 + 2*t*u + u**2 - 8*m**4)*(t - u) -
 4*(t + u + 4*m**2)*t**2)*c1(2) + 2*(t + u + 4*m**2)*(t - u + 2*m**2)*c3(2)*t)*(
(t + u)*m**2 + t*u)*(t + u)*u)*(t + u) - 3*(2*((t + u + 4*m**2)**2*(9*b2(2) + 6*
b2(1) + 4*b2(0)) + 27*(t + u + 4*m**2)*(t + u + 2*m**2)*(2*cf - nc)*(t + u)*c6(2
) + 27*(c1(2)*m**2 - 4)*(t + u)**2*nc + 27*((t + u)*c4(2) - b2(1))*(t + u + 4*m
**2)*(2*cf - nc)*(t + u)) - 9*((t + u + 4*m**2)*log(m**2/mur**2)**3*beta0 - 3*(t
 + u)*b5(2)*nc)*(t + u))*(t**2 + u**2 - 2*(t + u)*m**2)*((t + u)*m**2 + t*u)*u)*
t + 54*((((2*(t + u)*m**2 + t*u)*(t + u + 4*m**2)*(7*b1(2)*u + 2*b1u(2)*t) - (18
*m**2 + 2*t + 7*u)*(t + u)*b5(2)*t*u)*(t + u) - 16*((t + u + 4*m**2)*(t**2 + 2*t
*u + u**2)*(t + 7*u) - 7*(t + u)*(t - u)*t*u)*m**2)*((t + u)*m**2 + t*u) - (t + 
u + 4*m**2)*(t**2 + 2*t*u + u**2)*(t + u)*(t - u)*c1(1)*m**2*t*u)*(t + u))*(t + 
u + 4*m**2)*(t**2 + 2*t*u + u**2) - 648*(4*(t + u + 4*m**2)*(7*cf + nc) + (t + u
 - 8*m**2)*b5(2)*nc - (2*(b2(1) - 1) + b2(2))*(t + u + 4*m**2)*(2*cf - nc) + (2*
(3*c1(2)*m**2 - 5 - b5(1))*(t + u) + (t**2 + 2*t*u + u**2)*c1(1) + 24*m**2)*nc)*
((t + u)*m**2 + t*u)**2*(t + u)**3*m**2*t*u)*(nc - 3 - 2*cf) - (((((3*(2*((t + u
 + 4*m**2)*(3*b2(1) + 2*b2(0)) + 9*(t + u + 2*m**2)*(2*cf - nc)*(t + u)*c6(1) + 
9*((t + u)*c4(1) - b2(0))*(2*cf - nc)*(t + u)) + 9*(3*nc - 2 - 6*cf)*(t + u)*b2(
1) + 6*(5*nc - 2*nlf - 9*cf)*(t + u)*b5(1) + 4*(5*nc + nlf - 9*cf)*(t + u)*b5(0)
) + 8*(nlf + 1 + 14*nc + 54*cf)*(t + u))*(t + u + 4*m**2) + 27*((2*(c1(1)*m**2 -
 2) + b5(1))*(t + u)*nc - (t + u + 4*m**2)*log(m**2/mur**2)**2*beta0)*(t + u))*(
3*((t + u + 2*m**2)*c6(-1) + (t + u)*c4(-1))*(2*cf - nc) - (15*cf - 14*ln - 4*
lnu))*(t**2 + u**2 - 2*(t + u)*m**2)*((t + u)*m**2 + t*u)*u - 54*(((((t**2 + 3*u
**2 - 2*(t + u)*m**2)*((t + u)*m**2 + t*u)*(c4(1) - d2u(1)*u) - (t**2 + 2*t*u + 
u**2)*(t - u)*c1(0)*m**2)*u - 2*((2*m**2 - u)*(t + u) + 2*t*u)*((t + u)*m**2 + t
*u)*b1u(0) - ((c4(0) - d2u(0)*u)*(t + u) - 2*c3u(0)*u)*((t**2 - u**2)*m**2 + 2*t
**2*u)*u)*(t + u + 4*m**2) - 2*(((t + u)*t - 8*m**4)*c1(0) - (t - u)*b5(0))*((t 
+ u)*m**2 + t*u)*(t + u)*u)*(t + u) - 2*(4*(t + u + 4*m**2)*(t**2 + 2*t*u + u**2
)*m**2 + (2*m**2 + t)*(t + u)**2*b5(1)*u - (2*(t + u)*m**2 + t*u)*(t + u + 4*m**
2)*(t + u)*b1u(1))*((t + u)*m**2 + t*u))*(((t + u + 2*m**2)*c6(-1) + (t + u)*c4(
-1))*(2*cf - nc) + 2*(ln + 2*lnu) - 5*cf)*(t + u))*t - 27*((((2*((2*(t + u)*m**2
 + t*u)*(t + u + 4*m**2)*b1(1) - (2*m**2 + u)*(t + u)*b5(1)*t) + (3*t**2 + u**2 
- 2*(t + u)*m**2)*(t + u + 4*m**2)*(c4(1) - d2(1)*t)*t)*(t + u) - 16*((t + u + 4
*m**2)*(t**2 + 2*t*u + u**2) - (t + u)*(t - u)*t)*m**2)*((t + u)*m**2 + t*u) - (
(2*m**2 + t)*(t + u)*c1(0) - 2*c3(0)*t**2 + (c4(0) - d2(0)*t)*(t + u)*t)*((2*m**
2 - t)*(t + u) - (t**2 + u**2))*(t + u + 4*m**2)*(t + u)*t)*(7*((t + u + 2*m**2)
*c6(-1) + (t + u)*c4(-1))*(2*cf - nc) - (35*cf - 38*ln - 4*lnu)) - ((((t**2 + 2*
t*u + u**2 - 8*m**4)*(t - u) - 4*(t + u + 4*m**2)*t**2)*c1(1) + 2*(t + u + 4*m**
2)*(t - u + 2*m**2)*c3(1)*t)*(7*((t + u + 2*m**2)*c6(-1) + (t + u)*c4(-1))*(2*cf
 - nc) - (35*cf - 38*ln - 4*lnu)) - 2*(((t**2 + 2*t*u + u**2 - 8*m**4)*(t - u) +
 4*(t + u + 4*m**2)*u**2)*c1(1) + 2*(t + u + 4*m**2)*(t - u - 2*m**2)*c3u(1)*u)*
(((t + u + 2*m**2)*c6(-1) + (t + u)*c4(-1))*(2*cf - nc) + 2*(ln + 2*lnu) - 5*cf)
)*((t + u)*m**2 + t*u)*(t + u)*t)*(t + u)*u)*(t + u + 4*m**2)*(t**2 + 2*t*u + u
**2) + 216*(2*((3*c1(1)*m**2 - 1 - b5(0))*(t + u)*nc + 6*(t + u + 4*m**2)*cf) - 
(2*(b2(0) - 1) + b2(1))*(t + u + 4*m**2)*(2*cf - nc) + ((t**2 + 2*t*u + u**2)*c1
(0) + 24*m**2 + (t + u - 8*m**2)*b5(1))*nc)*(3*((t + u + 2*m**2)*c6(-1) + (t + u
)*c4(-1))*(2*cf - nc) - (15*cf - 14*ln - 4*lnu))*((t + u)*m**2 + t*u)**2*(t + u)
**3*m**2*t*u))*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*(t**2 + 2*t*u +
 u**2))*(t + u + 4*m**2)*(t + u) + (((4*(3*(((2*(9*((t + u + 4*m**2)*log(m**2/
mur**2)*beta0 - (t + u)*c1(0)*m**2*nc) - (19*(t + u) + 112*m**2)*nc) - 3*(2*(5*
nc - 2*nlf - 9*cf)*(t + u + 4*m**2) + 3*(t + u)*nc)*b5(0))*(t + u) - 3*(t + u + 
4*m**2)**2*b2(0))*(t + u + 4*m**2)*b2(0) + (9*(2*(t + u + 4*m**2)*log(m**2/mur**
2)*beta0 - (b5(0) + 2*c1(0)*m**2)*(t + u)*nc) - 2*(19*(t + u) + 112*m**2)*nc - 3
*(5*nc - 2*nlf - 9*cf)*(t + u + 4*m**2)*b5(0))*(5*nc - 2*nlf - 9*cf)*(t + u)**2*
b5(0)) + 2*((2*(9*((t + u + 4*m**2)*log(m**2/mur**2)*beta0 - (t + u)*c1(0)*m**2*
nc) - (19*(t + u) + 112*m**2)*nc) - 3*(2*(5*nc - 2*nlf - 9*cf)*(t + u + 4*m**2) 
+ 3*(t + u)*nc)*b5(0))*(t + u) - 2*(3*(t + u + 4*m**2)*b2(0) + (nlf + 1)*(t + u)
)*(t + u + 4*m**2))*(nlf + 1)*(t + u) + 9*((2*(9*((t + u + 4*m**2)*log(m**2/mur
**2)*beta0 - (t + u)*c1(0)*m**2*nc) - (19*(t + u) + 112*m**2)*nc) - 3*(2*(5*nc -
 2*nlf - 9*cf)*(t + u + 4*m**2) + 3*(t + u)*nc)*b5(0))*(t + u) - ((9*(2*cf - nc)
*(t + u)*c4(0) + 4*(nlf + 1))*(t + u) + 6*(t + u + 4*m**2)*b2(0))*(t + u + 4*m**
2))*(2*cf - nc)*(t + u)**2*c4(0) + 9*((2*(9*((t + u + 4*m**2)*log(m**2/mur**2)*
beta0 - (t + u)*c1(0)*m**2*nc) - (19*(t + u) + 112*m**2)*nc) - 3*(2*(5*nc - 2*
nlf - 9*cf)*(t + u + 4*m**2) + 3*(t + u)*nc)*b5(0))*(t + u) - ((2*(9*(2*cf - nc)
*(t + u)*c4(0) + 2*(nlf + 1)) + 9*(t + u + 2*m**2)*(2*cf - nc)*c6(0))*(t + u) + 
6*(t + u + 4*m**2)*b2(0))*(t + u + 4*m**2))*(t + u + 2*m**2)*(2*cf - nc)*(t + u)
*c6(0))*(t + u + 4*m**2) + (4*((9*(47*(t + u) + 224*m**2)*(t + u) - 784*(t + u +
 4*m**2)**2)*nc**2 + 9*(2*(19*(t + u) + 112*m**2)*nc - 9*(t + u + 4*m**2)*log(m
**2/mur**2)*beta0)*(t + u + 4*m**2)*log(m**2/mur**2)*beta0 + 9*(9*(2*(t + u + 4*
m**2)*log(m**2/mur**2)*beta0 - (t + u)*c1(0)*m**2*nc) - 2*(19*(t + u) + 112*m**2
)*nc)*(t + u)*c1(0)*m**2*nc) + 9*(9*(4*(t + u + 4*m**2)*log(m**2/mur**2)*beta0 -
 (b5(0) + 4*c1(0)*m**2)*(t + u)*nc) - 4*(19*(t + u) + 112*m**2)*nc)*(t + u)*b5(0
)*nc)*(t + u)**2 - 9*((4*((9*(2*cf - nc)*(t + u)*c4(0) + 2*(nlf + 1) + 9*(t + u 
+ 2*m**2)*(2*cf - nc)*c6(0))*(t + u) + 3*(t + u + 4*m**2)*b2(0)) + 9*(3*nc - 2 -
 6*cf)*(t + u)*b2(0))*(t + u + 4*m**2) - 2*(2*(9*((t + u + 4*m**2)*log(m**2/mur
**2)*beta0 - (t + u)*c1(0)*m**2*nc) - (19*(t + u) + 112*m**2)*nc) - 3*(2*(5*nc -
 2*nlf - 9*cf)*(t + u + 4*m**2) + 3*(t + u)*nc)*b5(0))*(t + u))*(3*nc - 2 - 6*cf
)*(t + u + 4*m**2)*(t + u)*b2(0))*(t**2 + u**2 - 2*(t + u)*m**2)*(t + u + 4*m**2
)*(t**2 + 2*t*u + u**2) + 72*(2*((2*((9*(2*cf - nc)*(t + u)*c4(0) + 2*(nlf + 1) 
+ 9*(t + u + 2*m**2)*(2*cf - nc)*c6(0))*(t + u) + 3*(t + u + 4*m**2)*b2(0)) + 9*
(3*nc - 2 - 6*cf)*(t + u)*b2(0) + 6*(5*nc - 2*nlf - 9*cf)*(t + u)*b5(0))*(t + u 
+ 4*m**2) - (9*(2*(t + u + 4*m**2)*log(m**2/mur**2)*beta0 - (b5(0) + 2*c1(0)*m**
2)*(t + u)*nc) - 2*(19*(t + u) + 112*m**2)*nc)*(t + u)) + 9*((t + u + 4*m**2)*(
b2(0) - 2)*(2*cf - nc) - (t + u - 8*m**2)*b5(0)*nc - 6*((t + u)*c1(0) + 4)*m**2*
nc)*(t + u))*((t + u + 4*m**2)*(b2(0) - 2)*(2*cf - nc) - (t + u - 8*m**2)*b5(0)*
nc - 6*((t + u)*c1(0) + 4)*m**2*nc)*((t + u)*m**2 + t*u)*(t + u)**3*m**2)*t*u - 
6*(2*((2*((t**2 + 3*u**2 - 2*(t + u)*m**2)*(t + u + 4*m**2)*(c4(0) - d2u(0)*u) -
 (18*m**2 + 2*t + 7*u)*(t + u)*b5(0)) + 7*(3*t**2 + u**2 - 2*(t + u)*m**2)*(t + 
u + 4*m**2)*(c4(0) - d2(0)*t))*(t + u)*t*u - 8*((t + u + 4*m**2)*(t**2 + 2*t*u +
 u**2)*(2*t + 7*u) - 5*(t + u)*(t - u)*t*u)*m**2)*(t + u + 4*m**2)*(27*b5(0)*cf 
- 15*b5(0)*nc + 6*b5(0)*nlf - 28*nc - 2*nlf - 2)*(t + u) + 3*(2*(4*((t + u + 4*m
**2)*(t**2 + 2*t*u + u**2)*(2*t + 7*u) - 5*(t + u)*(t - u)*t*u)*m**2 + (18*m**2 
+ 2*t + 7*u)*(t + u)**2*b5(0)*t*u) - (7*(3*t**2 + u**2 - 2*(t + u)*m**2)*(c4(0) 
- d2(0)*t) + 2*(t**2 + 3*u**2 - 2*(t + u)*m**2)*(c4(0) - d2u(0)*u))*(t + u + 4*m
**2)*(t + u)*t*u)*(2*(3*((t + u + 2*m**2)*c6(0) + (t + u)*c4(0))*(2*cf - nc)*(t 
+ u) + (t + u + 4*m**2)*b2(0))*(t + u + 4*m**2) + 3*((2*(c1(0)*m**2 - 1) + b5(0)
)*(t + u)*nc - 2*(t + u + 4*m**2)*log(m**2/mur**2)*beta0)*(t + u)) + 2*((2*(9*((
t + u + 4*m**2)*log(m**2/mur**2)*beta0 - (c1(0)*m**2 - 1)*(t + u)*nc) - 2*(nlf +
 1 + 14*nc)*(t + u + 4*m**2)) - 3*(2*(5*nc - 2*nlf - 9*cf)*(t + u + 4*m**2) + 3*
(t + u)*nc)*b5(0))*(t + u) - 6*(3*((t + u + 2*m**2)*c6(0) + (t + u)*c4(0))*(2*cf
 - nc)*(t + u) + (t + u + 4*m**2)*b2(0))*(t + u + 4*m**2))*(2*(t + u)*m**2 + t*u
)*(t + u + 4*m**2)*(7*b1(0)*u + 2*b1u(0)*t)*(t + u) - 72*(7*(2*((t + u)*m**2 + t
*u) - ((t - u)*c1(0) - 2*c3(0)*t)*(m**2 + t)*t - ((t + u)*m**2 + t*u)*b1(0) + ((
t + u)*m**2 - (t - u)*t)*(c4(0) - d2(0)*t)*t)*u + 2*(2*((t + u)*m**2 + t*u) + ((
t - u)*c1(0) + 2*c3u(0)*u)*(m**2 + u)*u - ((t + u)*m**2 + t*u)*b1u(0) + ((t + u)
*m**2 + (t - u)*u)*(c4(0) - d2u(0)*u)*u)*t)*((6*((t + u)*c1(0) + 4)*m**2 + (t + 
u - 8*m**2)*b5(0))*nc - (t + u + 4*m**2)*(b2(0) - 2)*(2*cf - nc))*(t + u)**2*m**
2 - 9*((2*((2*(t + u)*m**2 + t*u)*(t + u + 4*m**2)*(7*b1(0)*u + 2*b1u(0)*t) - (
18*m**2 + 2*t + 7*u)*(t + u)*b5(0)*t*u + (t**2 + 3*u**2 - 2*(t + u)*m**2)*(t + u
 + 4*m**2)*(c4(0) - d2u(0)*u)*t*u) + 7*(3*t**2 + u**2 - 2*(t + u)*m**2)*(t + u +
 4*m**2)*(c4(0) - d2(0)*t)*t*u)*(t + u) - 8*((t + u + 4*m**2)*(t**2 + 2*t*u + u
**2)*(2*t + 7*u) - 5*(t + u)*(t - u)*t*u)*m**2)*(3*nc - 2 - 6*cf)*(t + u + 4*m**
2)*(t + u)*b2(0) + ((2*(3*(3*((t + u + 2*m**2)*c6(0) + (t + u)*c4(0))*(2*cf - nc
)*(t + u) + (t + u + 4*m**2)*b2(0)) + 2*(nlf + 1 + 14*nc)*(t + u)) + 9*(3*nc - 2
 - 6*cf)*(t + u)*b2(0) + 6*(5*nc - 2*nlf - 9*cf)*(t + u)*b5(0))*(t + u + 4*m**2)
 + 9*((2*(c1(0)*m**2 - 1) + b5(0))*(t + u)*nc - 2*(t + u + 4*m**2)*log(m**2/mur
**2)*beta0)*(t + u))*(7*(((t**2 + 2*t*u + u**2 - 8*m**4)*(t - u) - 4*(t + u + 4*
m**2)*t**2)*c1(0) + 2*(t + u + 4*m**2)*(t - u + 2*m**2)*c3(0)*t) - 2*(((t**2 + 2
*t*u + u**2 - 8*m**4)*(t - u) + 4*(t + u + 4*m**2)*u**2)*c1(0) + 2*(t + u + 4*m
**2)*(t - u - 2*m**2)*c3u(0)*u))*(t + u)*t*u)*(t + u + 4*m**2)*(t + u)**3)*((t +
 u)*m**2 + t*u)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*(t**2 + 2*t*u 
+ u**2))*((t + u)*m**2 + t*u) + 108*(2*(((((t + u)*m**2 + (t - u)*u)*c4(0) + 2*(
m**2 + u)*c3u(0)*u - ((t + u)*m**2 + (t - u)*u)*d2u(0)*u)*(t + u + 4*m**2)*(t - 
u) - 2*((t + u)*b5(0) + 8*m**2 - (t + u + 4*m**2)*b1u(0))*((t + u)*m**2 + t*u) -
 ((4*(t + u + 4*m**2)*t*u - (t**2 + 2*t*u + u**2)*(t + u))*(m**2 + u) - 4*(t + u
)*m**2*u**2)*c1(0))*(2*((t + u + 4*m**2)*(m**2 + t)*b1(0) - 4*(2*m**2 + t)*m**2 
- ((3*t + u)*m**2 + (t + u)*t)*b5(0))*((t + u)*m**2 + t*u)*(t + u) - (t + u + 4*
m**2)*(m**2 + t)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*d2(0)*t**2 + ((((t + u)*m**
2 + t*u)*(t + u + 2*m**2) + (t + u + 4*m**2)*t**2)*(2*m**2 + t)*c1(0) + ((t + u)
*c4(0) - 2*c3(0)*t)*(t + u + 4*m**2)*(m**2 + t)*t)*(t + u)**2)*t*u - 2*(2*((t + 
u + 4*m**2)*(b1(0) - 2)*(m**2 + t) - (b5(0) - 2)*(2*m**2 + t)*t)*((t + u)*m**2 +
 t*u) + ((c4(0) - d2(0)*t)*(t + u) - 2*c3(0)*t)*(t + u + 4*m**2)*t**3 + (((t + u
)*m**2 + t**2)*(t + u + 4*m**2)*t + ((t + u)*m**2 + t*u)*(2*m**2 + t)*(t + u))*
c1(0)*t)*((((t + u)*m**2 + (t - u)*u)*(c4(0) - d2u(0)*u) + ((t - u)*c1(0) + 2*
c3u(0)*u)*(m**2 + u))*u - ((t + u)*m**2 + t*u)*(b1u(0) - 2))*(t + u + 4*m**2)*(t
**2 + 2*t*u + u**2)*m**2)*(t + u) + ((((((3*t + u)*m**2 + 2*t**2)*(t + u + 4*m**
2) + (2*m**2 + t)*(t + u)*t)*((t + u)*m**2 + t*u) + ((t + u)*m**2 + t**2)*(t + u
 + 4*m**2)*t**2)*(t + u)*c1(0) + 2*((((t + u)*m**2 + t*u)*(t + u + 4*m**2) - (2*
m**2 + t)*(t + u)*t)*((t + u)*m**2 + t*u)*b5(0) - ((t + 2*u)*t + (t + u)*m**2)*(
t + u + 4*m**2)*(m**2 + t)*(t + u)*c3(0)*t))*(t + u)*t + 2*(4*(((t + u)*m**2 + t
*u)*(t + u + 4*m**2) - (t - u)*t**2)*m**2 - (2*(t + u)*m**2 - (t - u)*t)*(t + u 
+ 4*m**2)*(m**2 + t)*b1(0))*((t + u)*m**2 + t*u)*(t + u) - (((t + u)*m**2 - 2*t
**2)*((t + u)*m**2 + t*u) - (t + u)*t**3)*(t + u + 4*m**2)*(c4(0) - d2(0)*t)*(t
**2 + 2*t*u + u**2)*t)*((2*((2*(t + u)*m**2 + t*u)*(t + u + 4*m**2)*b1u(0) - (2*
m**2 + t)*(t + u)*b5(0)*u) + (t**2 + 3*u**2 - 2*(t + u)*m**2)*(t + u + 4*m**2)*(
c4(0) - d2u(0)*u)*u)*(t + u) - 8*((t + u + 4*m**2)*(t**2 + 2*t*u + u**2) + (t + 
u)*(t - u)*u)*m**2 + (((t**2 + 3*u**2 - 2*(t - u)*m**2)*(t + u + 4*m**2) - 2*(t 
+ u)*(t - u)*m**2)*c1(0) + 2*(t + u + 4*m**2)*(t - u - 2*m**2)*c3u(0)*u)*(t + u)
*u) - ((2*(((3*t + u)*m**2 + (t + u)*t)*b5(0)*u - ((2*t + u)*m**2 + t*u)*(t + u 
+ 4*m**2)*b1u(0)) - (t**2 + u**2 - (t + u)*m**2)*(t + u + 4*m**2)*(c4(0) - d2u(0
)*u)*u)*(t + u) + 8*((t + u + 4*m**2)*(t**2 + 2*t*u + u**2) - (2*m**2 + u)*(t + 
u)*u)*m**2 - (((t**2 - 2*t*u + 5*u**2 - 8*m**2*t)*m**2 + t**3 + t**2*u + t*u**2 
+ u**3)*c1(0) + 2*(t + u + 4*m**2)*(t - u - m**2)*c3u(0)*u)*(t + u)*u)*(2*((((t 
+ u)*m**2 + t**2)*(t + u + 4*m**2) + ((t + u)*m**2 + t*u)*(t - u))*(t + u)*c1(0)
 - 2*(4*(2*m**2 + u) + (t - u)*b5(0))*((t + u)*m**2 + t*u) + (((c4(0) - d2(0)*t)
*(t**2 + 2*t*u + u**2) - 2*(t + u)*c3(0)*t)*t + 2*((t + u)*m**2 + t*u)*b1(0))*(t
 + u + 4*m**2))*m**2 - ((((c4(0) - d2(0)*t)*(t + u) - 2*c3(0)*t)*((t + u)*m**2 +
 t**2) + ((3*t - u)*m**2 + t**2)*(t + u)*c1(0))*t - 2*(b5(0)*t + 4*m**2 - (2*m**
2 + t)*b1(0))*((t + u)*m**2 + t*u))*(t + u + 4*m**2))*(t + u)**2*t + (2*(4*(2*(8
*t + 5*u)*m**2 + (4*t + 9*u)*t)*m**2 - ((8*t + 5*u)*m**2 + 4*t*u)*(t + u + 4*m**
2)*b1u(0)) - ((4*(t - u) - 5*m**2)*(t + u) + 10*u**2)*(t + u + 4*m**2)*(c4(0) - 
d2u(0)*u)*u + 2*(4*(t + u + 4*m**2)*t - 5*(t - u)*m**2)*b5(0)*u - ((2*(2*t**2 + 
3*u**2 - (4*t - u)*m**2)*(t + u + 4*m**2) - 5*(t + u)*(t - u)*m**2)*c1(0) + 2*(t
 + u + 4*m**2)*(4*(t - u) - 5*m**2)*c3u(0)*u)*u)*(((c4(0) - d2(0)*t)*t + (2*m**2
 + t)*c1(0))*(t + u) - 2*c3(0)*t**2)*((t + u)*m**2 + t*u)*(t + u + 4*m**2)*(t**2
 + 2*t*u + u**2)*(t + u)*t)*(t + u + 4*m**2)*(t**4 + 4*t**3*u + 6*t**2*u**2 + 4*
t*u**3 + u**4)*(t**2 + 2*t*u + u**2)*(t + u)**3)*u - 108*((((((t + u)*m**2 + (t 
- u)*u)*c4(0) + 2*(m**2 + u)*c3u(0)*u - ((t + u)*m**2 + (t - u)*u)*d2u(0)*u)*(t 
+ u + 4*m**2)*(t - u) - 2*((t + u)*b5(0) + 8*m**2 - (t + u + 4*m**2)*b1u(0))*((t
 + u)*m**2 + t*u) - ((4*(t + u + 4*m**2)*t*u - (t**2 + 2*t*u + u**2)*(t + u))*(m
**2 + u) - 4*(t + u)*m**2*u**2)*c1(0))*(((((t**2 + 2*t*u + u**2)*c1(0) - 16*m**2
)*(2*m**2 + u) + 2*(t + u + 2*m**2)*(t - u)*b5(0))*(t + u)*u - 2*(((t - u)*u + 2
*m**2*t)*(t + u)*b1u(0) - 4*(t**2 + 2*t*u + u**2)*m**2)*(t + u + 4*m**2))*((t + 
u)*m**2 + t*u) - (((c4(0) - d2u(0)*u)*(t + u) - 2*c3u(0)*u)*((t - u)*m**2 - u**2
) - ((2*m**2 + t)*(t + u)*m**2 + (2*m**2 + u)*u**2)*c1(0))*(t + u + 4*m**2)*(t**
2 + 2*t*u + u**2)*u)*u + 4*(((((t + u)*m**2 + t*u)*(2*m**2 + u)*(t + u) + ((t + 
u)*m**2 + u**2)*(t + u + 4*m**2)*u)*c1(0) + ((c4(0) - d2u(0)*u)*(t + u) - 2*c3u(
0)*u)*(t + u + 4*m**2)*u**2)*u - 2*(2*((t + u)*m**2 + t*u) + (b5(0)*u + 4*m**2)*
(2*m**2 + u) - (t + u + 4*m**2)*(m**2 + u)*b1u(0))*((t + u)*m**2 + t*u))*((((t +
 u)*m**2 + (t - u)*u)*(c4(0) - d2u(0)*u) + ((t - u)*c1(0) + 2*c3u(0)*u)*(m**2 + 
u))*u - ((t + u)*m**2 + t*u)*(b1u(0) - 2))*(t + u + 4*m**2)*(t**2 + 2*t*u + u**2
)*m**2 - 2*((2*((2*(t + u)*m**2 + t*u)*(t + u + 4*m**2)*b1u(0) - (2*m**2 + t)*(t
 + u)*b5(0)*u) + (t**2 + 3*u**2 - 2*(t + u)*m**2)*(t + u + 4*m**2)*(c4(0) - d2u(
0)*u)*u)*(t + u) - 8*((t + u + 4*m**2)*(t**2 + 2*t*u + u**2) + (t + u)*(t - u)*u
)*m**2 + (((t**2 + 3*u**2 - 2*(t - u)*m**2)*(t + u + 4*m**2) - 2*(t + u)*(t - u)
*m**2)*c1(0) + 2*(t + u + 4*m**2)*(t - u - 2*m**2)*c3u(0)*u)*(t + u)*u)*(((2*t -
 u - 2*m**2)*((t + u)*m**2 + t*u) - t**2*u)*(t + u + 4*m**2)*b1u(0) - 4*(((t + 3
*u)*t + 4*(t + u)*m**2)*t - ((t + u)*m**2 + t*u)*(t + u + 4*m**2))*m**2 - ((t**2
 - u**2)*t - 4*(t + u)*m**4 + (t**2 - 4*t*u - u**2)*m**2)*b5(0)*u)*((t + u)*m**2
 + t*u) + ((2*(((3*t + u)*m**2 + (t + u)*t)*b5(0)*u - ((2*t + u)*m**2 + t*u)*(t 
+ u + 4*m**2)*b1u(0)) - (t**2 + u**2 - (t + u)*m**2)*(t + u + 4*m**2)*(c4(0) - 
d2u(0)*u)*u)*(t + u) + 8*((t + u + 4*m**2)*(t**2 + 2*t*u + u**2) - (2*m**2 + u)*
(t + u)*u)*m**2 - (((t**2 - 2*t*u + 5*u**2 - 8*m**2*t)*m**2 + t**3 + t**2*u + t*
u**2 + u**3)*c1(0) + 2*(t + u + 4*m**2)*(t - u - m**2)*c3u(0)*u)*(t + u)*u)*(2*(
(((t + u)*m**2 + t*u)*(t - u) - ((t + u)*m**2 + u**2)*(t + u + 4*m**2))*(t + u)*
c1(0) + 2*(4*(2*m**2 + t) - (t - u)*b5(0))*((t + u)*m**2 + t*u) - (((c4(0) - d2u
(0)*u)*(t**2 + 2*t*u + u**2) - 2*(t + u)*c3u(0)*u)*u + 2*((t + u)*m**2 + t*u)*
b1u(0))*(t + u + 4*m**2))*m**2*u - (((c4(0) - d2u(0)*u)*(t + u) - 2*c3u(0)*u)*((
t + u)*m**2 + u**2)*u + 2*((2*m**2 + u)*b1u(0) - 4*m**2)*((t + u)*m**2 + t*u) - 
(2*((t + u)*m**2 + t*u)*b5(0) + ((t - 3*u)*m**2 - u**2)*(t + u)*c1(0))*u)*(t + u
 + 4*m**2)*t)*(t + u) + (2*(4*(2*(8*t + 5*u)*m**2 + (4*t + 9*u)*t)*m**2 - ((8*t 
+ 5*u)*m**2 + 4*t*u)*(t + u + 4*m**2)*b1u(0)) - ((4*(t - u) - 5*m**2)*(t + u) + 
10*u**2)*(t + u + 4*m**2)*(c4(0) - d2u(0)*u)*u + 2*(4*(t + u + 4*m**2)*t - 5*(t 
- u)*m**2)*b5(0)*u - ((2*(2*t**2 + 3*u**2 - (4*t - u)*m**2)*(t + u + 4*m**2) - 5
*(t + u)*(t - u)*m**2)*c1(0) + 2*(t + u + 4*m**2)*(4*(t - u) - 5*m**2)*c3u(0)*u)
*u)*(((c4(0) - d2u(0)*u)*u + (2*m**2 + u)*c1(0))*(t + u) - 2*c3u(0)*u**2)*((t + 
u)*m**2 + t*u)*(t + u + 4*m**2)*(t**2 + 2*t*u + u**2)*u)*(t + u) + (((((2*((2*(t
 + u)*m**2 + t*u)*(t + u + 4*m**2)*b1u(0) - (2*m**2 + t)*(t + u)*b5(0)*u) + (t**
2 + 3*u**2 - 2*(t + u)*m**2)*(t + u + 4*m**2)*(c4(0) - d2u(0)*u)*u)*(t + u) - 8*
((t + u + 4*m**2)*(t**2 + 2*t*u + u**2) + (t + u)*(t - u)*u)*m**2)*((2*(m**2 + u
)*(t + u) + (t - u)*m**2)*(t + u + 4*m**2) + 2*((t + 3*u)*m**2 + (t + u)*u)*t)*(
(t + u)*m**2 + t*u)*(t + u) + (((2*(m**2 + u)*(t + u) + (t - u)*m**2)*(t + u + 4
*m**2) + 2*((t + 3*u)*m**2 + (t + u)*u)*t)*((t + u)*m**2 + t*u)*(t + u)**2 + ((t
 + u + 4*m**2)*(t**2 + 2*t*u + u**2) + (t + u)*(t - u)*u)*(t + u + 4*m**2)*(t**2
 + 2*t*u + u**2)*m**2)*(((t**2 + 3*u**2 - 2*(t - u)*m**2)*(t + u + 4*m**2) - 2*(
t + u)*(t - u)*m**2)*c1(0) + 2*(t + u + 4*m**2)*(t - u - 2*m**2)*c3u(0)*u)*u)*(t
 + u) + ((2*((2*(t + u)*m**2 + t*u)*(t + u + 4*m**2)*b1u(0) - (2*m**2 + t)*(t + 
u)*b5(0)*u) + (t**2 + 3*u**2 - 2*(t + u)*m**2)*(t + u + 4*m**2)*(c4(0) - d2u(0)*
u)*u)*((t + u + 4*m**2)*(t**2 + 2*t*u + u**2) + (t + u)*(t - u)*u)*(t + u) - 8*(
(2*(t + u + 4*m**2)*(t**2 + 2*t*u + u**2) + (t + u)*(t - u)*u)*(t + u)*(t - u)*u
 + (t + u + 4*m**2)**2*(t**2 + 2*t*u + u**2)**2)*m**2)*(t + u + 4*m**2)*(t**2 + 
2*t*u + u**2)*m**2)*c1(0) + ((2*((2*(t + u)*m**2 + t*u)*(t + u + 4*m**2)*b1u(0) 
- (2*m**2 + t)*(t + u)*b5(0)*u) + (t**2 + 3*u**2 - 2*(t + u)*m**2)*(t + u + 4*m
**2)*(c4(0) - d2u(0)*u)*u)*(t + u) - 8*((t + u + 4*m**2)*(t**2 + 2*t*u + u**2) +
 (t + u)*(t - u)*u)*m**2 + (((t**2 + 3*u**2 - 2*(t - u)*m**2)*(t + u + 4*m**2) -
 2*(t + u)*(t - u)*m**2)*c1(0) + 2*(t + u + 4*m**2)*(t - u - 2*m**2)*c3u(0)*u)*(
t + u)*u)*((((m**2 + 4*u)*(t + u) - 2*u**2)*((t + u)*m**2 + t*u) - (t**2 + 2*t*u
 + u**2)*m**2*t)*(c4(0) - d2u(0)*u) + 2*(((t + u)*m**2 + t*u)*(m**2 - 2*u) + (t 
+ u)*m**2*t)*c3u(0)*u)*(t + u + 4*m**2)*(t + u)**2)*u)*(t + u + 4*m**2)*(t**4 + 
4*t**3*u + 6*t**2*u**2 + 4*t*u**3 + u**4)*(t**2 + 2*t*u + u**2)*(t + u)**3*t)*t 
+ 513*(((((((3*t + u)*m**2 + 2*t**2)*(t + u + 4*m**2) + (2*m**2 + t)*(t + u)*t)*
((t + u)*m**2 + t*u) + ((t + u)*m**2 + t**2)*(t + u + 4*m**2)*t**2)*(t + u)*c1(0
) + 2*((((t + u)*m**2 + t*u)*(t + u + 4*m**2) - (2*m**2 + t)*(t + u)*t)*((t + u)
*m**2 + t*u)*b5(0) - ((t + 2*u)*t + (t + u)*m**2)*(t + u + 4*m**2)*(m**2 + t)*(t
 + u)*c3(0)*t))*(t + u)*t + 2*(4*(((t + u)*m**2 + t*u)*(t + u + 4*m**2) - (t - u
)*t**2)*m**2 - (2*(t + u)*m**2 - (t - u)*t)*(t + u + 4*m**2)*(m**2 + t)*b1(0))*(
(t + u)*m**2 + t*u)*(t + u) - (((t + u)*m**2 - 2*t**2)*((t + u)*m**2 + t*u) - (t
 + u)*t**3)*(t + u + 4*m**2)*(c4(0) - d2(0)*t)*(t**2 + 2*t*u + u**2)*t)*((2*((2*
(t + u)*m**2 + t*u)*(t + u + 4*m**2)*b1(0) - (2*m**2 + u)*(t + u)*b5(0)*t) + (3*
t**2 + u**2 - 2*(t + u)*m**2)*(t + u + 4*m**2)*(c4(0) - d2(0)*t)*t)*(t + u) - 8*
((t + u + 4*m**2)*(t**2 + 2*t*u + u**2) - (t + u)*(t - u)*t)*m**2 + (((3*t**2 + 
u**2 + 2*(t - u)*m**2)*(t + u + 4*m**2) + 2*(t + u)*(t - u)*m**2)*c1(0) - 2*(t +
 u + 4*m**2)*(t - u + 2*m**2)*c3(0)*t)*(t + u)*t) + 2*((((t + u)*m**2 - (t - u)*
t)*c4(0) + 2*(m**2 + t)*c3(0)*t - ((t + u)*m**2 - (t - u)*t)*d2(0)*t)*(t + u + 4
*m**2)*(t - u) + 2*((t + u)*b5(0) + 8*m**2 - (t + u + 4*m**2)*b1(0))*((t + u)*m
**2 + t*u) + ((4*(t + u + 4*m**2)*t*u - (t**2 + 2*t*u + u**2)*(t + u))*(m**2 + t
) - 4*(t + u)*m**2*t**2)*c1(0))*(2*((t + u + 4*m**2)*(m**2 + t)*b1(0) - 4*(2*m**
2 + t)*m**2 - ((3*t + u)*m**2 + (t + u)*t)*b5(0))*((t + u)*m**2 + t*u)*(t + u) -
 (t + u + 4*m**2)*(m**2 + t)*(t**3 + 3*t**2*u + 3*t*u**2 + u**3)*d2(0)*t**2 + ((
((t + u)*m**2 + t*u)*(t + u + 2*m**2) + (t + u + 4*m**2)*t**2)*(2*m**2 + t)*c1(0
) + ((t + u)*c4(0) - 2*c3(0)*t)*(t + u + 4*m**2)*(m**2 + t)*t)*(t + u)**2)*(t + 
u)*t**2 + (2*(4*((6*t + u)*u + 2*(5*t + 2*u)*m**2)*m**2 - ((5*t + 2*u)*m**2 + t*
u)*(t + u + 4*m**2)*b1(0) - ((m**2 - u)*(t + u) - 6*m**2*t)*b5(0)*t) + ((t - u +
 5*m**2)*(t + u) - 10*t**2)*(t + u + 4*m**2)*(c4(0) - d2(0)*t)*t - (2*(((4*t - u
)*m**2 + 5*t**2)*c1(0) - (t - u + 5*m**2)*c3(0)*t)*(t + u + 4*m**2) - (t + u - m
**2)*(t + u)*(t - u)*c1(0))*t)*(((c4(0) - d2(0)*t)*t + (2*m**2 + t)*c1(0))*(t + 
u) - 2*c3(0)*t**2)*((t + u)*m**2 + t*u)*(t + u + 4*m**2)*(t**2 + 2*t*u + u**2)*(
t + u)*t + ((((((t**2 + 2*t*u + u**2)*m**2 + (t + u)*t**2)*(c4(0) - d2(0)*t) - 2
*((t + u)*m**2 + t**2)*c3(0)*t + ((3*t**2 + 2*t*u - u**2)*m**2 + (t + u)*t**2)*
c1(0))*t - 2*(b5(0)*t + 4*m**2 - (2*m**2 + t)*b1(0))*((t + u)*m**2 + t*u))*((((t
 + u)*m**2 - 2*t**2)*(c4(0) - d2(0)*t) - 2*(m**2 + t)*c1(0)*t)*(t + u + 4*m**2) 
+ (2*(t + u + 4*m**2)*c3(0)*t - (t + u)*(t - u)*c1(0))*m**2 + 2*(4*(2*m**2 + u) 
+ (t - u)*b5(0) - (t + u + 4*m**2)*b1(0))*m**2)*t**2 - 4*(((((t + u)*m**2 + t**2
)*(t + u + 4*m**2)*t + ((t + u)*m**2 + t*u)*(2*m**2 + t)*(t + u))*c1(0) + ((c4(0
) - d2(0)*t)*(t + u) - 2*c3(0)*t)*(t + u + 4*m**2)*t**2)*t - 2*(2*((t + u)*m**2 
+ t*u) + (b5(0)*t + 4*m**2)*(2*m**2 + t) - (t + u + 4*m**2)*(m**2 + t)*b1(0))*((
t + u)*m**2 + t*u))*((((t + u)*m**2 - (t - u)*t)*(c4(0) - d2(0)*t) - ((t - u)*c1
(0) - 2*c3(0)*t)*(m**2 + t))*t - ((t + u)*m**2 + t*u)*(b1(0) - 2))*m**2)*(t + u 
+ 4*m**2) - 2*((((t + u)*m**2 + t**2)*(t + u + 4*m**2) + ((t + u)*m**2 + t*u)*(t
 - u))*(t + u)*c1(0) - 2*(4*(2*m**2 + u) + (t - u)*b5(0))*((t + u)*m**2 + t*u) +
 (((c4(0) - d2(0)*t)*(t**2 + 2*t*u + u**2) - 2*(t + u)*c3(0)*t)*t + 2*((t + u)*m
**2 + t*u)*b1(0))*(t + u + 4*m**2))*((((t + u)*m**2 - 2*t**2)*(c4(0) - d2(0)*t) 
- 2*(m**2 + t)*c1(0)*t)*(t + u + 4*m**2) + (2*(t + u + 4*m**2)*c3(0)*t - (t + u)
*(t - u)*c1(0))*m**2 + 2*(4*(2*m**2 + u) + (t - u)*b5(0) - (t + u + 4*m**2)*b1(0
))*m**2)*m**2*t**2)*(t + u)**3)*(t + u + 4*m**2)*(t**4 + 4*t**3*u + 6*t**2*u**2 
+ 4*t*u**3 + u**4)*(t**2 + 2*t*u + u**2)*(t + u)**3*u**2))/(81*((t + u)*m**2 + t
*u)**2*(t + u + 4*m**2)**3*(t + u)**12*t**2*u**2)$

